The relationship of SMBHs and host galaxies at $z<4$ in the deep optical variability-selected AGN sample in the COSMOS field

We present the study on the relationship between SMBHs and their host galaxies using our variability-selected AGN sample ($i_\mathrm{AB} \leq 25.9,\ z \leq 4.5$) constructed from the HSC-SSP Ultra-deep survey in the COSMOS field. We estimated the BH mass ($M_\mathrm{BH}=10^{5.5-10}\ M_{\odot}$) based on the single-epoch virial method and the total stellar mass ($M_\mathrm{star}=10^{10-12}\ M_{\odot}$) by separating the AGN component with SED fitting. We found that the redshift evolution of the BH-stellar mass ratio ($M_\mathrm{BH}/M_\mathrm{star}$) depends on the $M_\mathrm{BH}$ which is caused by the no significant correlation between $M_\mathrm{BH}$ and $M_\mathrm{star}$. Variable AGNs with massive SMBHs ($M_\mathrm{BH}>10^{9}\ M_{\odot}$) at $1.5<z<3$ show considerably higher BH-stellar mass ratios ($>\sim1\%$) than the BH-bulge ratios ($M_\mathrm{BH}/M_\mathrm{bulge}$) observed in the local universe for the same BH range. This implies that there is a typical growth path of massive SMBHs which is faster than the formation of the bulge component as final products seen in the present day. For the low-mass SMBHs ($M_\mathrm{BH}<10^{8}\ M_{\odot}$) at $0.5<z<3$, on the other hand, variable AGNs show the similar BH-stellar mass ratios with the local objects ($\sim 0.1\%$) but smaller than those observed at $z > 4$. We interpret that host galaxies harboring less massive SMBHs at intermediate redshift have already acquired sufficient stellar mass, although high-z galaxies are still in the early stage of galaxy formation relative to those at the intermediate/local universe.

==> 10appen.tex <==
%  \begin{table}[ht]
%  \centering
%  \caption{The classification of varAGN}
%   \label{class}
%    \begin{tabular}{cccc}
%     \hline \hline
%    Name  & X-ray & Virial mass & $\chi^2_\mathrm{red}$ \\
% %   &(1)&(2)&(3)\\
%    \hline
%    X-det varAGN ($\lambda_\mathrm{Edd}=0.1$)   & o & x & $ <5$ \\
%    X-det varAGN & o & o & $ <10 $ \\
%    X-undet varAGN ($\lambda_\mathrm{Edd}=0.1$)   & x & x  &$ <5 $\\
%    X-undet varAGN  & x & o  & $ <10 $\\
% \hline
%   \end{tabular}
%   %  \begin{tablenotes}
%   % \item[]Column (1)(2) (3)
%   % \end{tablenotes}
%  \end{table}



% \begin{figure}[htbp]
% \begin{center}
% \includegraphics[width=70mm]{fig-luminosity.pdf}
% \caption{Comparison of the bolometric luminosity $\Lbol$ converted from hard X-ray and SED fitting results (accretion luminosity). The black solid line show that the same bolometric luminosity and the gray shaded area represents a 10 times difference.}
% \label{luminosity}
% \end{center}
% \end{figure}



% \begin{table}[h]
% \centering
% \caption{Galaxy Data}
% \begin{tabular}{cccccccccccc}
% \hline
% Galaxy & Type & $\sigma$ (km/s) & $N_s$ & $\log(L/L_\odot)$ & $\log(M/M_\odot)$ & $M/L$ & $r_e$ (arcsec) & $M_{\bullet}$ ($M_\odot$) & $M_{\bullet,\mathrm{ref}}$ & $\Delta M_{\bullet,\mathrm{ref}}$ & Reference \\
% \hline
% M 32 & E2 & 0.805 & 7 & 5.10 & -19.45 & -16.64 & 2.816 & $9.05 \pm 0.10$ & $2.45(1.43 - 3.46) \times 10^6$ & 77 $\pm$ 3 & 1 0 1 & van den Bosch + 2010 \\
% NGC 1316 & E4 & 20.95 & 1 & 5.32 & -26.29 & -23.38 & 2.910 & $11.84 \pm 0.09$ & $1.69(1.39 - 1.97) \times 10^8$ & 226 $\pm$ 9 & 1 0 0 & Nowak + 2008 \\
% NGC 1332 & E6 & 22.66 & 2 & 7.05 & -24.73 & -21.58 & 3.159 & $11.27 \pm 0.09$ & $1.47(1.27 - 1.68) \times 10^9$ & 328 $\pm$ 9 & 1 0 0 & Rusli + 2011 \\
% NGC 1374 & E0 & 19.57 & 1 & 8.16 & -23.30 & -20.43 & 2.874 & $10.65 \pm 0.09$ & $5.90(5.39 - 6.51) \times 10^8$ & 167 $\pm$ 03 & 1 0 1 & Rusli + 2013 \\
% NGC 1399 & E1 & 20.85 & 1 & 6.31 & -25.29 & -22.43 & 2.863 & $11.50 \pm 0.09$ & $8.81(4.35 - 17.81) \times 10^8$ & 315 $\pm$ 03 & 1 1 0 & see notes \\
% NGC 1407 & E0 & 29.00 & 2 & 6.46 & -25.87 & -22.89 & 2.980 & $11.74 \pm 0.09$ & $4.65(4.24 - 5.38) \times 10^9$ & 276 $\pm$ 2 & 1 1 1 & Rusli + 2013 \\
% NGC 1550 & E1 & 52.50 & 9 & 8.77 & -24.87 & -21.89 & 2.974 & $11.33 \pm 0.09$ & $3.87(3.16 - 4.48) \times 10^9$ & 270 $\pm$ 10 & 1 1 1 & Rusli + 2013 \\
% NGC 2778 & E2 & 23.44 & 2 & 9.51 & -22.34 & -19.39 & 2.955 & $10.26 \pm 0.09$ & $1.45(0.00 - 2.91) \times 10^7$ & 175 $\pm$ 8 & 1 0 1 & Schulze + 2011 \\
% NGC 2960 & E2 & 67.1 & 9 & 9.78 & -24.36 & -21.30 & 3.068 & $11.06 \pm 0.09$ & $1.08(1.03 - 1.12) \times 10^7$ & 166 $\pm$ 16 & 3 0 0 & Kuo + 2011 \\
% NGC 3091 & E3 & 53.02 & 9 & 8.09 & -25.54 & -22.56 & 2.980 & $11.61 \pm 0.09$ & $3.72(3.21 - 3.83) \times 10^9$ & 297 $\pm$ 12 & 1 1 1 & Rusli + 2013 \\
% NGC 3377 & E5 & 10.99 & 2 & 7.16 & -23.06 & -20.08 & 2.980 & $10.50 \pm 0.09$ & $1.78(0.85 - 2.72) \times 10^8$ & 145 $\pm$ 7 & 1 0 1 & Schulze + 2011 \\
% NGC 3379 & E1 & 10.70 & 2 & 6.27 & -23.88 & -21.01 & 2.867 & $10.91 \pm 0.09$ & $4.16(3.12 - 5.20) \times 10^8$ & 206 $\pm$ 10 & 1 1 1 & van den Bosch + 2010 \\
% NGC 3607 & E1 & 22.65 & 2 & 6.99 & -24.79 & -21.92 & 2.872 & $11.26 \pm 0.09$ & $1.37(0.90 - 1.82) \times 10^8$ & 229 $\pm$ 11 & 1 1 0 & G¨ultekin + 2009b \\
% NGC 3608 & E1 & 22.75 & 2 & 7.62 & -24.17 & -21.19 & 2.980 & $11.01 \pm 0.09$ & $4.65(3.66 - 5.64) \times 10^8$ & 182 $\pm$ 9 & 1 1 1 & Schulze + 2011 \\
% NGC 3842 & E1 & 92.2 & 9 & 8.84 & -25.99 & -23.01 & 2.980 & $11.77 \pm 0.09$ & $9.09(6.28 - 11.43) \times 10^9$ & 270 ± 27 & 1 1 1 & McConnell + 2012 \\
% NGC 4261 & E2 & 32.36 & 2 & 6.94 & -25.62 & -22.64 & 2.980 & $11.65 \pm 0.09$ & $5.29(4.21 - 6.36) \times 10^8$ & 315 ± 15 & 2 1 0 & Ferrarese + 1996 \\
% NGC 4291 & E2 & 26.58 & 2 & 8.42 & -23.72 & -20.76 & 2.954 & $10.85 \pm 0.09$ & $9.78(6.70 - 12.86) \times 10^8$ & 242 ± 12 & 1 1 1 & Schulze + 2011 \\
% NGC 4374 & E1 & 18.51 & 1 & 5.75 & -25.60 & -22.62 & 2.980 & $11.62 \pm 0.09$ & $9.25(8.38 - 10.23) \times 10^8$ & 296 ± 14 & 2 1 0 & Walsh + 2010 \\
% NGC 4382 & E2 & 17.88 & 1 & 5.76 & -25.51 & -22.53 & 2.980 & $11.51 \pm 0.09$ & $1.30(0.00 - 22.4 ) \times 10^7$ & 182 ± 5 & 1 1 0 & G¨ultekin + 2011 \\
% NGC 4459 & E2 & 16.01 & 1 & 7.15 & -23.88 & -20.91 & 2.975 & $10.88 \pm 0.09$ & $6.96(5.62 - 8.29) \times 10^7$ & 167 ± 8 & 2 0 0 & Sarzi + 2001 \\
% NGC 4472 & E2 & 16.72 & 1 & 4.97 & -26.16 & -23.18 & 2.980 & $11.84 \pm 0.09$ & $2.54(2.44 - 3.12) \times 10^9$ & 300 ± 7 & 1 1 1 & Rusli + 2013 \\
% NGC 4473 & E5 & 15.25 & 1 & 7.16 & -23.77 & -20.89 & 2.874 & $10.85 \pm 0.09$ & $0.90(0.45 - 1.35) \times 10^8$ & 190 ± 9 & 1 0 1 & Schulze + 2011 \\
% M 87 & E1 & 16.68 & 1 & 5.27 & -25.85 & -22.87 & 2.980 & $11.72 \pm 0.09$ & $6.15(5.78 - 6.53) \times 10^9$ & 324+28 -12 & 1 1 1 & Gebhardt + 2011 \\
% NGC 4486A & E2 & 18.36 & 1 & 9.49 & -21.83 & -18.85 & 2.980 & . . . & $10.04 \pm 0.09$ & $1.44(0.92 - 1.97) \times 10^7$ & 111 ± 5 & 1 0 0 & Nowak + 2007 \\
% NGC 4486B & E0 & 16.26 & 1 & 10.39 & -20.67 & -17.69 & 2.980 & $9.64 \pm 0.10$ & $6. (4. - 9. ) \times 10^8$ & 185 ± 9 & 1 0 0 & Kormendy + 1997 \\
% NGC 4649 & E2 & 16.46 & 1 & 5.49 & -25.61 & -22.63 & 2.980 & $11.64 \pm 0.09$ & $4.72(3.67 - 5.76) \times 10^9$ & 380 ± 19 & 1 1 1 & Shen+Gebhardt 2010 \\
% NGC 4697 & E5 & 12.54 & 1 & 6.37 & -24.13 & -21.33 & 2.799 & $10.97 \pm 0.09$ & $2.02(1.52 - 2.53) \times 10^8$ & 177 ± 8 & 1 0 1 & Schulze + 2011 \\
% NGC 4751 & E6 & 32.81 & 2 & 8.24 & -24.38 & -21.22 & 3.158 & $11.16 \pm 0.09$ & $2.44(2.07 - 2.56) \times 10^9$ & 355 ± 14 & 1 0 1 & Rusli + 2013 \\
% NGC 4889 & E4 & 102.0 & 9 & 8.41 & -26.64 & -23.63 & 3.007 & $12.09 \pm 0.09$ & $2.08(0.49 - 3.66) \times 10^10$ & 347 ± 5 & 1 1 1 & McConnell + 2012 \\
% NGC 5077 & E3 & 38.7 & 9 & 8.22 & -24.74 & -21.66 & 2.949 & $11.28 \pm 0.09$ & $8.55(4.07 - 12.93) \times 10^8$ & 222 ± 11 & 2 1 0 & De Francesco + 2008 \\
% NGC 5128 & E & 3.62 & 6 & 3.49 & -24.34 & -21.36 & 2.980 & $11.05 \pm 0.09$ & $5.69(4.65 - 6.73) \times 10^7$ & 150 ± 7 & 1 1 0 & Cappellari + 2009 \\
% NGC 5516 & E3 & 55.3 & 9 & 8.31 & -25.47 & -22.50 & 2.970 & $11.60 \pm 0.09$ & $270 ± 27$ & 1 1 1 & McConnell + 2012 \\
% NGC 4261 & E2 & 32.36 & 2 & 6.94 & -25.62 & -22.64 & 2.980 & $11.65 \pm 0.09$ & $5.29(4.21 - 6.36) \times 10^8$ & 315 ± 15 & 2 1 0 & Ferrarese + 1996 \\
% NGC 4291 & E2 & 26.58 & 2 & 8.42 & -23.72 & -20.76 & 2.954 & $10.85 \pm 0.09$ & $9.78(6.70 - 12.86) \times 10^8$ & 242 ± 12 & 1 1 1 & Schulze + 2011 \\
% NGC 4374 & E1 & 18.51 & 1 & 5.75 & -25.60 & -22.62 & 2.980 & $11.62 \pm 0.09$ & $9.25(8.38 - 10.23) \times 10^8$ & 296 ± 14 & 2 1 0 & Walsh + 2010 \\
% NGC 4382 & E2 & 17.88 & 1 & 5.76 & -25.51 & -22.53 & 2.980 & $11.51 \pm 0.09$ & $1.30(0.00 - 22.4 ) \times 10^7$ & 182 ± 5 & 1 1 0 & G¨ultekin + 2011 \\
% NGC 4459 & E2 & 16.01 & 1 & 7.15 & -23.88 & -20.91 & 2.975 & $10.88 \pm 0.09$ & $6.96(5.62 - 8.29) \times 10^7$ & 167 ± 8 & 2 0 0 & Sarzi + 2001 \\
% NGC 4472 & E2 & 16.72 & 1 & 4.97 & -26.16 & -23.18 & 2.980 & $11.84 \pm 0.09$ & $2.54(2.44 - 3.12) \times 10^9$ & 300 ± 7 & 1 1 1 & Rusli + 2013 \\
% NGC 4473 & E5 & 15.25 & 1 & 7.16 & -23.77 & -20.89 & 2.874 & $10.85 \pm 0.09$ & $0.90(0.45 - 1.35) \times 10^8$ & 190 ± 9 & 1 0 1 & Schulze + 2011 \\
% M 87 & E1 & 16.68 & 1 & 5.27 & -25.85 & -22.87 & 2.980 & $11.72 \pm 0.09$ & $6.15(5.78 - 6.53) \times 10^9$ & 324+28 -12 & 1 1 1 & Gebhardt + 2011 \\
% NGC 4486A & E2 & 18.36 & 1 & 9.49 & -21.83 & -18.85 & 2.980 & . . . & $10.04 \pm 0.09$ & $1.44(0.92 - 1.97) \times 10^7$ & 111 ± 5 & 1 0 0 & Nowak + 2007 \\
% NGC 4486B & E0 & 16.26 & 1 & 10.39 & -20.67 & -17.69 & 2.980 & $9.64 \pm 0.10$ & $6. (4. - 9. ) \times 10^8$ & 185 ± 9 & 1 0 0 & Kormendy + 1997 \\
% NGC 4649 & E2 & 16.46 & 1 & 5.49 & -25.61 & -22.63 & 2.980 & $11.64 \pm 0.09$ & $4.72(3.67 - 5.76) \times 10^9$ & 380 ± 19 & 1 1 1 & Shen+Gebhardt 2010 \\
% NGC 4697 & E5 & 12.54 & 1 & 6.37 & -24.13 & -21.33 & 2.799 & $10.97 \pm 0.09$ & $2.02(1.52 - 2.53) \times 10^8$ & 177 ± 8 & 1 0 1 & Schulze + 2011 \\
% NGC 4751 & E6 & 32.81 & 2 & 8.24 & -24.38 & -21.22 & 3.158 & $11.16 \pm 0.09$ & $2.44(2.07 - 2.56) \times 10^9$ & 355 ± 14 & 1 0 1 & Rusli + 2013 \\
% NGC 4889 & E4 & 102.0 & 9 & 8.41 & -26.64 & -23.63 & 3.007 & $12.09 \pm 0.09$ & $2.08(0.49 - 3.66) \times 10^10$ & 347 ± 5 & 1 1 1 & McConnell + 2012 \\
% NGC 5077 & E3 & 38.7 & 9 & 8.22 & -24.74 & -21.66 & 2.949 & $11.28 \pm 0.09$ & $8.55(4.07 - 12.93) \times 10^8$ & 222 ± 11 & 2 1 0 & De Francesco + 2008 \\
% NGC 5128 & E & 3.62 & 6 & 3.49 & -24.34 & -21.36 & 2.980 & $11.05 \pm 0.09$ & $5.69(4.65 - 6.73) \times 10^7$ & 150 ± 7 & 1 1 0 & Cappellari + 2009 \\
% NGC 5516 & E3 & 55.3 & 9 & 8.31 & -25.47 & -22.50 & 2.970 & $11.60 \pm 0.09$ & $3.69(2.65 - 3.79) \times 10^9$ & 328 ± 11 & 1 1 1 & Rusli + 2013 \\
% NGC 5576 & E3 & 25.68 & 2 & 7.83 & -24.23 & -21.29 & 2.939 & $11.00 \pm 0.09$ & $2.73(1.94 - 3.41) \times 10^8$ & 183 ± 9 & 1 1 0 & G¨ultekin + 2009b \\
% NGC 5845 & E3 & 25.87 & 2 & 9.11 & -22.97 & -19.73 & 3.238 & $10.57 \pm 0.09$ & $4.87(3.34 - 6.40) \times 10^8$ & 239 ± 11 & 1 0 1 & Schulze + 2011 \\
% NGC 6086 & E & 138.0 & 9 & 9.97 & -25.74 & -22.84 & 2.884 & $11.69 \pm 0.09$ & $3.74(2.59 - 5.50) \times 10^9$ & 318 ± 2 & 1 1 1 & McConnell + 2011b \\
% NGC 6251 & E1 & 108.4 & 9 & 9.03 & -26.18 & -23.18 & 2.998 & . . . & $11.88 \pm 0.09$ & $6.14(4.09 - 8.18) \times 10^8$ & 290 ± 14 & 2 1 0 & Ferrarese + 1999 \\
% NGC 6861 & E4 & 28.71 & 2 & 7.71 & -24.60 & -21.42 & 3.179 & $11.25 \pm 0.09$ & $2.10(2.00 - 2.73) \times 10^9$ & 389 ± 3 & 1 0 1 & Rusli + 2013 \\
% NGC 7052 & E3 & 70.4 & 9 & 8.57 & -25.70 & -22.86 & 2.841 & $11.61 \pm 0.10$ & $3.96(2.40 - 6.72) \times 10^8$ & 266 ± 13 & 2 1 0 & van der Marel + 1998b \\
% NGC 7619 & E3 & 53.85 & 2 & 8.03 & -25.65 & -22.83 & 2.821 & $11.65 \pm 0.09$ & $2.30(2.19 - 3.45) \times 10^9$ & 292 ± 5 & 1 1 1 & Rusli + 2013 \\
% NGC 7768 & E4 & 116.0 & 9 & 9.34 & -26.00 & -23.19 & 2.811 & $11.75 \pm 0.09$ & $1.34(0.93 - 1.85) \times 10^9$ & 257 ± 26 & 1 1 1 & McConnell + 2012 \\
% \hline
% \end{tabular}
% \end{table}






==> 5dis.tex <==
\section{Discussion}
%\newcommand{\Rnum}[1]{\setcounter{num}{#1} \Roman{num}}
% \newcommand{\rnum}[1]{\setcounter{num}{#1} \roman{num}}
% \newcounter{num}
% \setcounter{num}{4} 
% \subsection{Search for the low-mass SMBH using the optical variability selection}
% Regarding the no spectroscopy varAGNs,,,
% In this paper, we provided the $\MBH-\Mstar$ relation over the wide $\MBH$ range at $z<3.5$ using the variability-selected AGNs.
% the potential for its existence persists in our sample.
% Assuming that the $\MBH-\Mbulge$ correlation have already shown at intermediate redshifts, the BH-bulge mass ratio may have higher value (e.g., $\MBH/\Mbulge\sim-1.5$) than local one considering that this hypothesis can be explained by the contribution of the disk component on the BH-stellar mass ratio for all BH mass ranges.
% \subsection{Redshift evolution of the BH-bulge mass ratio in massive SMBH}
% If the BH-stellar mass ratios across over the wide BH mass range ($5<\MBH/\Ms<10$) at intermediate redshift align with those in the local universe, it would be simply interpreted that SMBHs and their host galaxies have already co-evolved and these ratios can be explained by the disk contribution.
% However, i

In the AGNs with massive SMBHs ($9\leq\MBH/\Ms<10$) at the intermediate redshift, the average BH-stellar mass ratio (red dashed line in Figure \ref{s-ratio-bin}) is higher than that in the local universe (red upper triangle in Figure \ref{s-ratio-bin}), which means that massive SMBHs ($9\leq\MBH/\Ms<10$) follow a faster growth path rather than co-evolve with their host galaxies.
This indicates that the host galaxies have not yet acquired sufficient stellar mass, and at least their bulge components are still in the growth process (if the bulge mass had already acquired sufficient mass as seen in the $\MBH-\Mbulge$ relation in the local universe, the average BH-stellar mass ratio would be expected to be below -2). 
Then, we can interpret that the $\MBH - \Mbulge$ relation for massive SMBHs ($9\leq\MBH/\Ms<10$) evolves with redshift. 
From HST observations of the CANDELS field, \citet{mortlock2013redshift} showed the fraction of the spheroidal galaxies increase from $z=3$ to $z=1$ with a sample of massive galaxies with $\Mstar>10^{10} \Ms$ \citep[see also][]{tasca2014zcosmos}.
\citet{croton2006evolution} showed the redshift evolution of the $\MBH-\Mbulge$ relation using a model in which the bulge mass grows through the disruption of disks and starbursts during mergers.
However, the BH-stellar mass ratios in massive SMBHs show little variation and no significant redshift evolution between intermediate redshift and at $z>4$ \citep[e.g.,][]{izumi2019subaru,pensabene2020alma}, which could be due to the large disk contribution or the possibility that galaxies with massive SMBHs have already accumulated similar bulge masses at intermediate redshift.
Considering that high-z galaxies tend to be small size compared to those in the local universe \citep[e.g.,][]{labbe2023uncover,costantin2023expectations}, the disk contribution is seem to be relatively small at high-z.
% Since high-z AGNs often found in compact host galaxies, as reported in recent JWST observations \citep[e.g.,][]{labbe2023uncover}, the disk contribution is seem to be small at high-z.
We also inferred from their relatively large BH-stellar mass ratios that these massive SMBHs are expected to be in ETGs where the bulge contribution is significant.

% \subsection{Redshift evolution of the BH-bulge mass ratio in less massive SMBH}
Regarding the less massive SMBHs ($6\leq\MBH/\Ms<9$), would the $\MBH-\Mbulge$ relation show the redshift evolution?
% We also consider whether the $\MBH-\Mbulge$ relation for less massive SMBHs ($6\leq\MBH/\Ms<9$) shows redshift evolution or not. 
% Our interpretation 
The first idea is that, similar to the massive SMBHs ($9\leq\MBH/\Ms<10$), the $\MBH - \Mbulge$ relation for less massive SMBHs also evolves with redshift. 
Since the BH-stellar mass ratio remains relatively constant from the intermediate redshift to the local universe, host galaxies with less massive SMBHs at intermediate redshift have already gained significant stellar mass, while likely possessing larger disk contribution compared to those in the local universe.
% In this case, the host galaxies with less-massive SMBHs are expected to be LTGs with a large contribution of the disk component compared to the galaxies with massive SMBHs.
% Since the BH-stellar mass ratio does not change significantly between the local universe and intermediate redshift, the host galaxies with less-massive SMBHs at the intermediate redshift have acquired sufficient stellar mass, and they may have large disk component compared to the those in the local universe within the context of the redshift evolution of the BH-bulge mass ratio.
Therefore, in the BH-bulge redshift evolution, the galaxies with more massive SMBHs are likely to be ETGs, whereas those with less massive SMBHs tend to be spiral galaxies similar to the SMBH mass dependence of the galaxy morphology in the local universe \citep[e.g.,][]{beifiori2012correlations}.
% This is consistent with many observational studies.
% (Further discussion start)さらに、disk成分はbulge成分とは反対に、赤方偏移進化をすることで、the BH-stellar mass ratioが一定に保つことができる。\citet{tasca2014zcosmos}は、$z<1$ において the evolution of the light in bulges and discs を示している。ここではdisk stellar massがbulge成分に寄与することでtotal stellar mass を一定に保つことが可能にしている。（finish） 
Based on this idea, the large BH-stellar mass ratio in less massive SMBHs at high-z \citep[e.g.,][]{harikane2023jwst,maiolino2023jades} is explained by the reason that the bulge component is not adequately formed compared to those in the local universe.
% Furthermore, the larger values in the BH-bulge ratio at high-z, than those in the local universe, suggest that the contribution of the disk component is also smaller at high-z.
% allows for the interpretation that the reason the BH-stellar mass ratio in less-massive SMBHs differs between high redshift and the intermediate redshift (or in the loacl universe) is due to the fact that at high redshift, not only the bulge but also the disk component is less formed and less massive.

As an another idea, we consider that the $\MBH-\Mbulge$ relation for less massive SMBHs ($6\leq\MBH/\Ms<9$) does not evolve with redshift. 
Assuming the constant value of the BH-bulge ratio beyond the local universe, SMBHs and their host galaxies have already co-evolved and these ratios can be explained by the disk contribution.
The constant value of the BH-bulge ratio means that no significant variation of the BH-stellar mass ratio, which is consistent with the previous studies \citep[e.g.,][]{sun2015evolution,suh2020no} and also with our result.

However, \citet{pacucci2023jwst} shows that the $\MBH-\Mstar$ relation with low-mass SMBH range $\MBH/\Ms<{8.5}$ at $z>4$ deviates significantly from the local relation which is not due to selection effects.
The deviations of the $\MBH-\Mstar$ relation are also seen between at the intermediate redshift ($z<3$) and at the high-z ($z>4$) from our results (see Figure \ref{bh-st} or \ref{s-ratio-bin}).
Then, we support that the $\MBH-\Mbulge$ relation for the wide BH mass range ($6<\MBH/\Ms<10$) shows the redshift evolution to explain the high BH-stellar mass ratio at high-z.
Since JWST has allowed us to understand the morphology even at intermediate redshifts \citep[e.g.,][]{conte2023jwst}, we may be able to test the scenario by accurately separating the bulge and disk components through the AGN decomposition analysis using our variability sample.
% of galaxy formation scenario.
% The constancy of the BH-bulge ratio beyond the local universe aligns well with previous studies suggesting that the BH-stellar mass ratio at intermediate redshift does not evolve with redshift. 
% しかし、SMBH の質量が大きいAGNにおいて、近傍のBH-bulge 関係を超えている傾向にある、私たちの結果を含めて。
% But why is there redshift evolution of the BH-bulge mass ratio only for the massive SMBHs ($9\leq\MBH/\Ms<10$)?
% Also, why are the BH-stellar ratios at intermediate and high redshifts different?
% We considered that this idea is challenging for the following reasons: First, it fails to explain why there is redshift evolution of the BH-bulge mass ratio only for the massive SMBHs ($9\leq\MBH/\Ms<10$) ; second, it is difficult to determine when the BH-stellar mass ratio shows redshift evolution in the range of less massive SMBHs ($6\leq\MBH/\Ms<9$).
% Thus, we suggest that the BH-bulge mass ratio for all SMBH ranges shows the redshift evolution.


% \citet{croton2006evolution}ではbulge massは、合体中のthe disruption of disks and starburstsによって成長するモデルで、the $\MBH-\Mbulge$ relationが赤方偏移進化することを示している。さらにこのシナリオは,less-massive SMBHにおけるthe BH-stellar mass ratioが高赤方偏移と中間/近傍の宇宙におけて違う理由が、高赤方偏移ではbulgeだけでなくdisk成分も質量が少なく形成されていないためである解釈することができる。
% 別の解釈としてless massive SMBH ($6\leq\MBH/\Ms<9$)における $\MBH-\Mbulge$ relation が赤方偏移とともに進化していない場合を述べる。私たちは、以下の理由によりこの解釈は難しいと結論づけた。第一に何故赤方偏移進化しているか説明することができないこと、第二に、サンプルの限界からどこからless massive SMBHにおいてthe BH-stellar mass ratioが赤方偏移進化しているか把握できないからである。
% \subsection{How bulge and disk components evolve into the local relation}
% \subsection{do not read this section}
% The redshift evolution of the BH-bulge mass ratio supports the rapid SMBH growth scenario. 
% This is likely due to the effective AGN feedback suppressing star formation in the host galaxy. The question then arises: when and how do these galaxies form bulge and disk mass similar to those in the local universe? 
% While the AGNs with massive SMBH/small host is currently under debate, in the local universe, such objects with massive SMBH/small host are extremely rare and considered candidates for Red Nuggets, such as NGC1277, MRK1216, and PGC032873 \citep{van2012over,yildirim2015mrk}.
% Red Nuggets are galaxies with very high central density composed mostly of old, red stars. 
% \citep{van2005recent} have shown that Red Nuggets are formed through 'dry mergers' between gas-poor, bulge-dominated galaxies.
% Although, the AGNs with massive SMBH/small host at the intermediate redshift are thought to be the progenitors of those in the local universe, considering many of these objects will eventually evolve into the established $\MBH-\Mbulge$ relation seen in the local universe, it's necessary to increase the bulge stellar mass.
% Generally, merging galaxies and clumpy disk galaxies are more prevalent beyond the local universe, suggesting that the bulge could grow through mergers and the transformation of disk into bulge.
% \citet{croton2006evolution} showed a model where the bulge mass grows through the disruption of disks and starbursts during mergers, demonstrating that the $\MBH-\Mbulge$ relation evolves with redshift. 
% Since JWST has allowed us to understand the morphology even at intermediate redshifts \citep[e.g.,][]{conte2023jwst}, we may be able to test the scenario by accurately separating the bulge and disk components through the AGN decomposition analysis.


% To understand the evolution of SMBHs and their host galaxies into the local relation within the context of the redshift evolution of the BH-bulge mass ratio, it is necessary to consider how the bulge and disk components acquire sufficient stellar mass.


% g since galaxies have already shown at intermediate redshifts, the BH-bulge mass ratio may have higher value (e.g., $\MBH/\Mbulge\sim-1.5$) than local one considering that this hypothesis can be explained by the contribution of the disk component on the BH-stellar mass ratio for all BH mass ranges.
% The evolution of the $\MBH-\Mbulge$ relation has also been shown by the semi-analytic model of \citet{cattaneo2005active,croton2006evolution}.
% It can be inferred that the galaxy hosting massive SMBHs ($\MBH>10^8\ \Ms$) tend to be early-type galaxies, while those with less massive SMBHs ($\MBH<10^8\ \Ms$) tend to be late-type galaxies.
% However, the higher BH-bulge mass ratio at the intermediate redshift means that the bulge component has been forming compared to those with same SMBH mass in the present day.
% Considering the consistency of the BH-stellar mass ratio in the BH mass range $\MBH<10^9\ \Ms$, it is plausible that the bulge to disk mass ratio also evolves with redshift when compared at the same stellar mass range.
% SMBHs grow faster than the host galaxies compared to the present day.

% Yet, it does not resolve the problem of how the BH-stellar mass ratios in $9 \leq \MBH/\Ms < 10$ differ between the local universe and intermediate/high redshift.
% Considering many of these overmassive objects will eventually evolve into the established $\MBH-\Mbulge$ relation seen in the local universe, it's necessary to trigger events that increase only the stellar mass such as the dust-poor galaxy mergers.

% Recent observations by Subaru, ALMA and JWST have found the massive SMBHs (small host galaxies) at $z>4$ \citep[e.g.,][]{izumi2019subaru,pensabene2020alma}.
% Moreover, \citet{pacucci2023jwst} shows that the $\MBH-\Mstar$ relation with low-mass SMBH range $\MBH/\Ms<{8.5}$ at $z>4$ deviates significantly from the local relation which is not due to selection effects.
% % Many high-z AGN studies \citep[e.g.,][]{izumi2019subaru,pensabene2020alma} show that massive SMBHs (small host galaxies) are 
% The deviations of the $\MBH-\Mstar$ relation are also seen between at the intermediate redshift ($z<3$) and at the high-z ($z>4$) from our results (see Figure \ref{bh-st} or \ref{s-ratio-bin}).
% Then, we suggest that at high-z, the host galaxy is still in an early stage of galaxy formation, with only the core region around the galactic center being formed. 
% Subsequently, the disk component of the host galaxy begins its formation, evolving progressively from high-z to low-z.
% High-z AGNs often found in compact host galaxies, as reported in recent observations \citep[e.g.,][]{labbe2023uncover}, may be interpreted within this framework of galaxy formation scenario.

% Furthermore, we examine the alignment between model predicted and observed results in the evolution of the SMBHs and their host galaxies.
% Furthermore, model the trend of the increasing BH-stellar mass ratio with redshift is also suggested by 
% The two-phase model developed by \citet{Mo2023twophasemodel} have shown the similar evolutionary path, .

% Finally, we mention the SMBH-galaxy evolutionary pathway.
% From our sample and other local/high-z AGN sample, some objects have over weight SMBH compared to the local relation, others have almost same mass ratio of SMBH to the host galaxy.
% We can see the significant difference of the mass ratio particularly in the low-mass SMBH range ($6\leq\MBH/\Ms<8$) as discuss above.

% we support the SMBH
%our sampleは銀河形態に優位なバイアスはない、渦巻銀河と楕円銀河の割合
%normal 銀河の形態よりvariability-selected AGNsは対称的。
%IR-selected AGNsはdisk銀河が主要、一方でvariability-selected AGNは楕円銀河が主要の可能性。
% It's noted that AGNs with such compact host galaxies are frequently reported at high-z \citep[e.g.][]{labbe2023uncover}. 
% このセクションでは、赤方偏移とSMBH質量範囲によってBH-stellar関係が変化するか議論をする。
%私たちの中間赤方偏移サンプルと high-zのBH-stellar mass ratioについて比較する。 
% $\MBH=10^{8-10}\ \Ms$ のAGNは、ground-based telescopeによって検出されており、私たちのサンプルと同様に、z=6-8においても高いBH-stellar mass ratio(-1 to -2.5)を示し、赤方偏移進化が見られない事が示唆される。最近JWSTによって検出されたz=4-6のAGNは、$\MBH=10^{6-8}\ \Ms$ のSMBH質量であり、高いBH-stellar mass ratio(-1 to -2.5)を示した。$\MBH=10^{6-8}\ \Ms$ のSMBH質量のAGNは低赤方偏移z<1とhigh-zで値が増加し、赤方偏移進化していることが考えられる。これはhigh-zにおいて、母銀河は十分に成長していない段階であり、銀河中心に近いコア部分のみが形成されている状態である。high-zには、このようなコンパクトな母銀河を持つAGNが観測されている。よって私たちは、high-zからlow-zにかけて、母銀河のdisk成分が形成されて銀河進化していくシナリオを提案する。
%私たちのサンプルが近傍におけるBH-bulge関係に進化する可能性について議論する。BH-stellar 関係が無相関ということはBH-bulge関係に相関がない可能性が高い、なぜならbulge
% ground-based telescopeのAGN
% The specific Black Hole Accretion Rate (sBHAR) is a dimensionless quantity that represents the black hole accretion rate (BHAR $=(1-\eta)\Lbol/\eta c^2$) normalized by the black hole's own mass ($\MBH$) where we assume that energy conversion factor $\eta$ equals to 0.1 \citep[e.g.,][]{gruzinov1998radiative}. It provides a measure of how rapidly a black hole is growing in comparison to its current size.
% The specific star formation rate sSFR ($=\mathrm{SFR}/\Mstar$) is a key parameter in studies of galaxy evolution. 
% It allows for a comparison of the star-forming activity of galaxies of different sizes.
% To investigate how SMBHs and the host galaxies are evolving and interact with each other, we use the specific accretion rate sBHAR ($=\mathrm{BHAR}/\MBH$) and the specific star formation rate sSFR ($=\mathrm{SFR}/\Mstar$).

% To investigate how SMBHs and galaxies at intermediate redshifts evolve to the $\MBH-\Mbulge$ seen in the local universe, we present the $\mathrm{sBHAR/sSFR}$ - $\MBH/\Mstar$ plane shown in the Figure \ref{s-ratio}.
% Circle and star markers represent X-det varAGN and X-undet varAGN respectively.
% When sBHAR and sSFR are equal, it means that the $\MBH/\Mstar$ ratio is unchanged and growing together.
% The AGN plotted in the upper region ($\mathrm{sBHAR>sSFR}$) indicates that the BH is growing faster than the galaxy, leading to the increase of the $\MBH/\Mstar$ ratio. 
% For the lower region ($\mathrm{sBHAR<sSFR}$), on the contrary, the large star-forming of the host galaxy provides the decrease of the $\MBH/\Mstar$ ratio. 
% Redder (bluer) markers indicate more (less) massive SMBH.
% From the top panel, we can see that the lower mass SMBHs have a lower $\MBH/\Mstar$ ratio with a higher sBHAR/sSFR ratio, while massive SMBHs tend to have a higher $\MBH/\Mstar$ ratio with a lower sBHAR/sSFR ratio.
% % This trend can be interpreted that 
% Given that the magnitude of $\MBH/\Mstar$ ratio can somewhat predict galaxy morphology, this result suggests that galaxies evolve from late-type to early-type associated with the SMBH growth.
% The fraction $\MBH/\Mstar$ in X-det varAGN and X-undet varAGN growing for 100 Myr at the constant sBHAR and sSFR is plotted in the bottom panel.
% We can see that the varAGN with a low mass SMBH ($\MBH<10^7 \Ms$) shifted to the around the local $\MBH-\Mstar$ relation (blue dashed line), on the other hand, varAGN with a massive SMBH ($\MBH>10^8 \Ms$) shifted only a little and remain in a larger fraction even than the local $\MBH-\Mbulge$ relation.
% 母銀河に比べて中心BHが大きく成長した天体はRed Nuggets候補と考えられており、中心密度が非常に高く星形成が宇宙初期にほとんど終了してしまい赤い星が多く存在している銀河であり、高赤方偏移ほど多く観測されているものの近傍宇宙では観測例が少ない\citep[e.g.,][]{}。
% Considering that such overmassive SMBHs are observed more frequently at higher redshifts but less frequently in the local universe, it is suggested that most intermediate/high redshift AGNs with large ratios must undergo dry-merger or rapid star formation events in order to grow to the $\MBH-\Mbulge$ relation observed in the local universe.



% \begin{figure}[htbp]
% \begin{center}
% \includegraphics[width=80mm]{fig-s-ratio-ev.pdf}
% \caption{The co-evolution diagram of SMBHs and galaxies : The color gradient shows the distribution of $\MBH$ in X-det varAGN and X-undet varAGN sample. The red and blue dashed lines represent the $\MBH/\Mbulge$ ratio and $\MBH/\Mstar$ ratio in the bulge and stellar mass of $10^{11}\ \Ms$ in the local universe \citep{kormendy2013coevolution,reines2015relations}. The horizontal gray line shows that the specific SMBH accretion rate is equal to the specific SFR. The fraction of $\MBH/\Mstar$ after evolving for 100Myr at the constant sBHAR and sSFR is shown in the bottom panel.}
% \label{s-ratio}
% \end{center}
% \end{figure}

% Comparison with other selection,,,(Roman High Laitude Time Domain Survey)

\subsection{X-undet AGN}\label{xundet}
In this section, we discuss a subset of 50 AGNs in the optical variability sample. These sources are difficult to detect in the Chandra, although they are distinguished as X-ray sources by X-ray stacking analysis.
% X-ray stacking analysis reveals that X-ray undetected AGN in optical variability selected sample are the significant X-ray sources.
Despite AGN being too faint to be detected by X-rays, the optical variable sample contains 50 objects. 
The reason for the dark AGN in X-ray band could be low accretion rate or absorption by molecular dust. The former 
Eddington ratio
\subsection{varAGN showing Absorption Feature}
Among AGNs, there are Broad Absorption Lines (BAL) AGNs that exhibit the broad absorption line $\mathrm{FWHM} \ge 2000\ \mathrm{\kms}$ \citep{weymann1991comparisons}. In the X-ray and UV bands. In addition, depending on the velocity range, the min-BAL is used for absorption lines with $500\ \mathrm{\kms}\leq\mathrm{FWHM}<2000\ \mathrm{\kms}$, and the Narrow Absorption Lines (NAL). These absorption lines are thought to be caused primarily by outflow from the central nucleus and are characterized by shifted absorption lines \citep{elvis2000structure}. Systems with BALs are $\sim20\%$ of common AGNs \citep{knigge2008intrinsic,hewett2003frequency}.
\citet{vito2018no} reported that there is no evidence for a strong anti-correlation between X-ray suppression and Eddington ratio in BALQSOs sample. Instead, the strength of the BAL features appears to be a better tracer of $\Delta\aox$ than the Eddington ratio. 
\citet{page2016x} argued that X-ray absorption features related to the degree of ultraviolet absorption in C IV 1550 Å, appear to be ubiquitous in BALQSOs, but X-ray weakness is not. 


  


\begin{table*}[t]
 \centering
 \caption{varAGN showing Absorption Feature}
  \label{Absorp}
   \begin{tabular}{ccccc}
    \hline \hline
   
  ID&Line & $\Delta V_\mathrm{out}$ & $v_\mathrm{out}$  &HR  \\
  &&[$10^3\ \mathrm{km\ s^{-1}}$]&[$10^3\ \mathrm{km\ s^{-1}}$]&\\
  (1)&(2)&(3)&(4)&(5)\\
   \hline 
   \multicolumn{5}{c}{BALAGNs ($2\leq \Delta V_\mathrm{out}$)}\\
  *269 &$\Cfour$  & 3.2 & -4.9 &0.29 \\
  280&$\Cfour$&4.5, 2.1&-8.8, -0.3&0.31\\
  *295&$\Mgtwo$ & 3.1 & -2.1 &0.18 \\
    
  \hline
  \multicolumn{5}{c}{min-BALAGNs ($0.5\leq \Delta V_\mathrm{out} < 2$)}\\
  77&$\Cfour$&0.6, 0.4&0.3, 0.3&-0.12\\
  150 &$\Cfour$  & 0.8 & 1.0&-0.14\\
  151 &$\Cfour$  & 0.6 & 0.0&-0.36\\
  172 &$\Mgtwo$  & 1.1 & -1.4&-0.41\\
  266 &$\Cfour$ & 1.1 & -1.4&-0.04\\
  297&$\Mgtwo$&1.0, 0.3&-0.0, 0.8&-0.22\\
  312&$\Mgtwo$& 2.4 & -13.9&-0.22\\
    *313&$\Cfour$& 1.8 & -2.1&0.16\\
  *417&$\Cfour$& 1.1 & 1.6&0.05 \\
  (426)&$\Mgtwo$& 1.5 & 0.0&-0.27 \\
  \hline
  \multicolumn{5}{c}{NALAGNs ($\Delta V_\mathrm{out} \leq 0.5$)}\\
  212&$\Mgtwo$&0.5, 0.3&-0.8, -0.1&-0.09\\
  251&$\Mgtwo$&0.2, 0.2&-1.3, -0.5&-0.24\\
  256&$\Mgtwo$&0.4, 0.3&-0.1, -0.9&-0.20\\
  289&$\Mgtwo$&0.3, 0.3&-0.5, 0.3&0.38\\
  342&$\Cfour$&0.4, 0.3&-0.5, -0.1&0.27\\
  *377&$\Mgtwo$&0.4, 0.4&-0.8, -0.1&0.08\\
  *431&$\Cfour$&0.5, 0.2&-0.5, 0.0&-0.04\\

\hline
  \end{tabular}
  \begin{tablenotes}
  \item[]Column (1) varAGN ID listed in \citep{kimura_properties_2020} (2) Absorption Line 1:$\Mgtwo$, 2:$\Cfour$, 3:$\Hb$, 4:$\Ha$ (3) Absorption Velocity Width of FWHM (4) Outflow velocity (5) X-ray Hardness ratio \citep{park2006bayesian}.
  \end{tablenotes}
 \end{table*}
 \clearpage


==> Yamada2.tex <==
\section{Discuusion}

We here discuss the possible interpretation of our results in the previous section in terms of co-evolution of SMBHs and their host galaxies.
Our findings reveal the absence of a significant correlation between $\MBH$ and $\Mstar$, although it is not unclear whether a correlation exists between $\MBH$ and $\Mbulge$ at intermediate redshift, similar to that in the local universe \citep[e.g.,][]{kormendy2013coevolution}.

Firstly, we consider that the BH-stellar mass ratios with massive SMBHs ($9\leq\MBH/\Ms<10$) at the intermediate redshift show quite large values. 
In the local universe, most SMBHs in this mass range are typically found in giant elliptical galaxies with small disk contribution.
In Figure \ref{s-ratio-bin}, the red dashed line shows the average value, $\mathrm{log}\ (\MBH/\Mstar)$=$-1.5$, for the 7 objects at $1.5 < z < 3$, which is much larger than the BH-bulge ratio, $\mathrm{log}\ (\MBH$/$\Mbulge)$=$-2.2$ in the local universe for the same BH mass range \citep[e.g.,][]{kormendy2013coevolution}.
The presence of such large BH-stellar mass ratios implies that there is a typical growth path of massive SMBHs which is faster than the formation of stars in the associated bulges/spheroids as final products yet to reach the canonical mass ratio in the end.
% The presence of overmassive BHs even at intermediate redshift implies that the growth of stellar components occurs later than their observed epoch.
% At the intermediate redshift, the host galaxies with massive SMBHs have not yet acquired sufficient stellar mass, and at least their bulge components are still growing.
% If the bulge component acquires sufficient mass as observed in the $\MBH-\Mbulge$ relation in the local universe, the average BH-stellar mass ratio would be -2.2, which is further decreased when considering the disk contribution. 
% % In our sample, the $\MBH - \Mbulge$ relation for massive SMBHs ($10^9\leq\MBH/\Ms<10^{10}$) shows redshift evolution from the intermediate redshift to the local universe. 
At the higher redshift, $z>4$, \cite{izumi2019subaru} and \cite{pensabene2020alma} found that the BH-dynamical mass ratios also show the similar large value, $\mathrm{log}\ (\MBH/\Mdyn)\ge-2$.  Our results suggests that such overmassive BH appears not only at the very early universe where the gas cooling efficiency is high but also at the intermediate redshift at $1.5<z<3$.
\citet{pacucci2024redshift} show the interpretation of the overmassive BHs with the assumption that black hole mass growth is regulated by the quasar's output, and the stellar mass growth is also quenched by it. 
This process works at high redshift when the host galaxies are physically small, and the accretion duty cycle is high, but a runaway process brings the originally overmassive system towards the local BH to stellar mass relation once the condition of suppressing star-formation is broken. This may explain the behavior of overmassive BH objects.
% However, the BH-stellar mass ratios in massive SMBHs show little variation and no significant redshift evolution between intermediate redshift and at $z>4$ \citep[e.g.,][]{izumi2019subaru,pensabene2020alma}, which could be due to the large disk contribution or the possibility that galaxies with massive SMBHs have already accumulated similar bulge masses at intermediate redshift.

% We also inferred from their relatively large BH-stellar mass ratios that these massive SMBHs are expected to be in ETGs where the bulge contribution is significant.
% In fact, \citet{mortlock2013redshift} showed that the fraction of the spheroidal galaxies increase from $z=3$ to $z=1$ among the massive galaxies with $\Mstar>10^{10} \Ms$ \citep[see also][]{tasca2014zcosmos}.
% Considering that high-z galaxies tend to be small size compared to those in the local universe \citep[e.g.,][]{labbe2023uncover,costantin2023expectations}, the disk contribution is seem to be relatively small at high-z.
% In the local universe, hosts of the most of the SMBH in this mass range are giant elliptical galaxies. 
% In fact, \citet{mortlock2013redshift} showed that the fraction of the spheroidal galaxies increase from $z=3$ to $z=1$ among the massive galaxies with $\Mstar>10^{10} \Ms$ \citep[see also][]{tasca2014zcosmos}.
% How the early type galaxies increase their stellar mass after the formation of their central BH? The two-phase models \citep{oser2010two} with later growth of mass by successive dry mergers can explain the properties of local elliptical galaxies and their plausible progenitors at high-redshift simultaneously. 
% It is, however, puzzling how the very tight $\MBH-\Mbulge$ relation is constructed as their end product as seen in the local universe. 

We also consider the cases for less massive SMBHs with $10^7\leq\MBH/\Ms<10^9$ whose BH-stellar mass ratio do not appear to evolve significantly over the observed redshift range for the given BH mass.
Although, the nearly constant BH to stellar mass ratio over the redshift range may indicate that the BH and bulges always co-evolve in their formation history including the contribution of the disk components, this contrasts with the recent discovery of the less massive SMBH at the higher redshift, $4<z<7$ \citep[e.g.,][]{harikane2023jwst,maiolino2023jades}.
\citet{pacucci2023jwst} shows that the $\MBH-\Mstar$ relation with low-mass SMBH range $\MBH/\Ms<{8.5}$ at $z>4$ deviates significantly from the local relation which is not due to selection effects.
Therefore, we speculate that the BH-bulge ratios for less massive SMBHs in our sample also show high values similar to the massive SMBHs. 
Since the BH-stellar mass ratio remains relatively constant from the intermediate redshift to the local universe, host galaxies with less massive SMBHs at intermediate redshift have already acquired total stellar mass.
These galaxies likely have a larger disk contribution compared to their local universe counterparts and to galaxies hosting massive SMBHs at intermediate redshifts.
% while likely possessing larger disk contribution compared to those in the local universe and to overmassive BH host galaxies at the intermediate redshift.
The SMBH mass dependence of the galaxy morphology is also seen in the local universe \citep[e.g.,][]{beifiori2012correlations}.
In fact, \citet{mortlock2013redshift} showed that the fraction of the spheroidal galaxies increase from $z=3$ to $z=1$ among the massive galaxies with $\Mstar>10^{10} \Ms$ \citep[see also][]{tasca2014zcosmos}.
% In the perspective of the redshift evolution, the large BH-stellar mass ratio in less massive SMBHs at high-z \citep[e.g.,][]{harikane2023jwst,maiolino2023jades} is explained by the reason that the bulge and disk components are not adequately formed compared to those in the local universe.
\citet{croton2006evolution} investigated the evolution of $\MBH-\Mbulge$ relation in their semi-analytic simulation. They argue that if galaxy mergers are the primary drivers for both BH and bulge growth, one should expect the $\MBH-\Mbulge$ relation to evolve with redshift, with a larger black hole mass associated with a given bulge mass at earlier times relative to the present day. In this model, the growth of bulge mass is due to the disruption of the disks in merging events. 
This model with high BH feeding efficiency could explane the high BH-bulge mass ratios observed beyond the local universe.

% Since JWST has allowed us to understand the morphology even at intermediate redshifts \citep[e.g.,][]{conte2023jwst}, we are be able to confirm the redshift evolution of the $\MBH-\Mbulge$ by accurately separating the bulge and disk components through the AGN decomposition analysis using our variability sample.

==> bhst_latex_with_kimura.tex <==
\begin{longtable}{|c|c|c|c|c|c|c|}
\hline
\hline
varAGN ID & Redshift & $\MBH$ & $\Mstar$ & $\chi_\mathrm{red}$ \\
\hline
(1) & (2) & (3) & (4) & (5) \\
\hline
\endhead\hline\endfoot
1 & 1.618 & 8.6 $\pm$ 1.08 & 11.0 $\pm$ 0.71 & 2.3 \\
2 & 3.497 & 8.8 $\pm$ 0.16 & 11.5 $\pm$ 0.49 & 1.5 \\
7 & 1.964 & 8.5 $\pm$ 0.07 & 10.3 $\pm$ 0.15 & 3.4 \\
12 & 1.518 & 7.9 $\pm$ 0.19 & 10.8 $\pm$ 0.21 & 1.9 \\
15 & 1.609 & 7.7 $\pm$ 0.41 & 11.1 $\pm$ 0.59 & 1.3 \\
19 & 2.74 & 7.7 $\pm$ 0.22 & 10.1 $\pm$ 0.14 & 3.1 \\
20 & 1.099 & 8.5 $\pm$ 0.04 & 11.1 $\pm$ 0.59 & 2.8 \\
22 & 2.023 & 8.4 $\pm$ 0.56 & 10.8 $\pm$ 0.49 & 3.7 \\
23 & 0.827 & 7.0 $\pm$ 0.19 & 10.3 $\pm$ 0.84 & 2.1 \\
28 & 2.836 & 7.7 $\pm$ 0.18 & 10.8 $\pm$ 0.36 & 4.0 \\
28 & 2.83 & 8.7 $\pm$ 0.57 & 10.8 $\pm$ 0.27 & 2.3 \\
33 & 0.376 & 7.4 $\pm$ 0.12 & 10.8 $\pm$ 1.25 & 3.2 \\
34 & 0.657 & 7.8 $\pm$ 0.05 & 11.1 $\pm$ 0.75 & 1.7 \\
36 & 2.122 & 8.3 $\pm$ 0.15 & 11.3 $\pm$ 0.48 & 3.6 \\
37 & 1.223 & 8.1 $\pm$ 0.15 & 10.9 $\pm$ 0.66 & 2.3 \\
43 & 1.142 & 8.6 $\pm$ 0.09 & 11.1 $\pm$ 0.84 & 1.9 \\
44 & 1.447 & 8.3 $\pm$ 0.11 & 11.0 $\pm$ 0.81 & 4.2 \\
46 & 2.16 & 7.3 $\pm$ 0.8 & 11.0 $\pm$ 0.47 & 1.6 \\
47 & 1.571 & 8.2 $\pm$ 0.3 & 10.3 $\pm$ 0.09 & 3.6 \\
51 & 2.234 & 7.4 $\pm$ 0.36 & 10.8 $\pm$ 0.51 & 1.9 \\
58 & 2.367 & 8.3 $\pm$ 1.21 & 10.4 $\pm$ 0.5 & 1.2 \\
60 & 2.171 & 8.6 $\pm$ 0.69 & 10.7 $\pm$ 0.19 & 3.9 \\
61 & 2.28 & 8.8 $\pm$ 0.28 & 10.4 $\pm$ 0.04 & 2.9 \\
64 & 0.669 & 7.5 $\pm$ 0.09 & 10.7 $\pm$ 0.74 & 2.1 \\
66 & 2.283 & 8.3 $\pm$ 0.28 & 11.1 $\pm$ 0.74 & 2.8 \\
73 & 0.882 & 7.8 $\pm$ 0.11 & 10.7 $\pm$ 0.43 & 1.5 \\
78 & 1.512 & 8.5 $\pm$ 0.15 & 11.1 $\pm$ 0.97 & 4.2 \\
79 & 1.256 & 7.8 $\pm$ 0.11 & 11.3 $\pm$ 0.81 & 1.4 \\
83 & 2.155 & 8.7 $\pm$ 0.77 & 11.1 $\pm$ 0.41 & 2.5 \\
91 & 2.03 & 9.1 $\pm$ 0.11 & 10.9 $\pm$ 0.31 & 3.4 \\
92 & 1.714 & 7.8 $\pm$ 0.65 & 10.6 $\pm$ 0.25 & 1.6 \\
93 & 2.037 & 7.5 $\pm$ 0.23 & 10.2 $\pm$ 0.33 & 2.5 \\
95 & 1.931 & 7.8 $\pm$ 0.22 & 10.7 $\pm$ 0.36 & 2.6 \\
96 & 2.05 & 8.5 $\pm$ 0.15 & 11.0 $\pm$ 0.32 & 1.0 \\
99 & 2.068 & 8.4 $\pm$ 0.52 & 10.9 $\pm$ 0.85 & 3.4 \\
101 & 2.754 & 9.2 $\pm$ 0.1 & 10.9 $\pm$ 0.31 & 2.4 \\
105 & 2.053 & 8.7 $\pm$ 0.76 & 10.7 $\pm$ 0.57 & 2.1 \\
109 & 2.055 & 8.6 $\pm$ 0.1 & 10.8 $\pm$ 0.11 & 4.3 \\
113 & 1.759 & 7.5 $\pm$ 0.86 & 10.4 $\pm$ 0.68 & 1.6 \\
119 & 1.56 & 8.2 $\pm$ 0.33 & 11.2 $\pm$ 0.55 & 1.6 \\
121 & 2.027 & 8.0 $\pm$ 0.18 & 10.9 $\pm$ 0.28 & 2.3 \\
126 & 2.654 & 8.6 $\pm$ 0.19 & 10.7 $\pm$ 0.31 & 2.6 \\
128 & 0.904 & 7.8 $\pm$ 0.16 & 11.1 $\pm$ 0.88 & 2.9 \\
129 & 2.005 & 8.1 $\pm$ 1.09 & 11.0 $\pm$ 0.59 & 1.3 \\
130 & 2.23 & 8.4 $\pm$ 0.37 & 10.9 $\pm$ 0.61 & 2.6 \\
131 & 2.994 & 8.3 $\pm$ 0.51 & 11.1 $\pm$ 0.75 & 1.1 \\
132 & 2.611 & 9.9 $\pm$ 0.24 & 10.6 $\pm$ 0.1 & 2.5 \\
133 & 1.817 & 8.2 $\pm$ 0.08 & 10.2 $\pm$ 0.11 & 1.8 \\
134 & 2.483 & 8.0 $\pm$ 0.34 & 10.8 $\pm$ 0.31 & 3.4 \\
136 & 1.829 & 8.4 $\pm$ 0.24 & 11.5 $\pm$ 0.46 & 1.7 \\
138 & 1.841 & 8.2 $\pm$ 0.08 & 10.4 $\pm$ 0.33 & 4.6 \\
140 & 2.083 & 8.5 $\pm$ 0.37 & 11.0 $\pm$ 0.52 & 3.6 \\
142 & 2.04 & 8.5 $\pm$ 0.56 & 11.3 $\pm$ 0.5 & 1.4 \\
144 & 1.503 & 7.3 $\pm$ 0.57 & 10.4 $\pm$ 0.3 & 2.0 \\
147 & 1.936 & 8.5 $\pm$ 0.12 & 10.6 $\pm$ 0.16 & 3.3 \\
149 & 0.696 & 7.4 $\pm$ 0.28 & 10.7 $\pm$ 0.75 & 2.3 \\
152 & 2.653 & 8.9 $\pm$ 0.13 & 10.1 $\pm$ 0.14 & 3.7 \\
154 & 0.958 & 8.2 $\pm$ 0.42 & 11.1 $\pm$ 0.84 & 2.0 \\
155 & 1.836 & 8.0 $\pm$ 0.12 & 10.6 $\pm$ 0.15 & 3.8 \\
158 & 1.603 & 8.7 $\pm$ 1.22 & 11.1 $\pm$ 0.62 & 1.9 \\
160 & 1.589 & 8.2 $\pm$ 0.22 & 11.0 $\pm$ 0.64 & 2.7 \\
166 & 2.126 & 8.2 $\pm$ 0.66 & 11.0 $\pm$ 0.65 & 1.9 \\
168 & 2.167 & 8.4 $\pm$ 0.22 & 10.9 $\pm$ 0.28 & 1.6 \\
169 & 2.388 & 8.3 $\pm$ 0.64 & 10.7 $\pm$ 0.56 & 2.8 \\
170 & 2.276 & 8.8 $\pm$ 0.06 & 10.7 $\pm$ 0.19 & 3.8 \\
171 & 1.625 & 8.2 $\pm$ 0.33 & 11.4 $\pm$ 0.52 & 4.7 \\
172 & 1.679 & 9.2 $\pm$ 0.13 & 10.6 $\pm$ 0.74 & 4.7 \\
173 & 1.358 & 7.3 $\pm$ 0.56 & 10.3 $\pm$ 0.55 & 1.3 \\
174 & 1.661 & 8.4 $\pm$ 0.12 & 10.5 $\pm$ 0.22 & 3.2 \\
174 & 1.666 & 7.6 $\pm$ 0.12 & 10.7 $\pm$ 0.31 & 3.1 \\
176 & 1.817 & 7.6 $\pm$ 0.96 & 9.9 $\pm$ 0.6 & 3.3 \\
179 & 2.405 & 8.1 $\pm$ 0.49 & 10.9 $\pm$ 0.85 & 4.8 \\
184 & 3.499 & 8.3 $\pm$ 0.08 & 10.9 $\pm$ 0.46 & 2.4 \\
185 & 2.498 & 8.5 $\pm$ 0.06 & 10.3 $\pm$ 0.37 & 3.8 \\
186 & 2.131 & 8.3 $\pm$ 0.83 & 11.0 $\pm$ 0.78 & 2.3 \\
195 & 1.796 & 8.8 $\pm$ 0.14 & 10.6 $\pm$ 0.12 & 3.0 \\
196 & 1.406 & 8.1 $\pm$ 0.05 & 11.1 $\pm$ 0.63 & 2.3 \\
199 & 0.728 & 6.6 $\pm$ 0.31 & 10.9 $\pm$ 0.96 & 2.7 \\
203 & 1.258 & 8.4 $\pm$ 0.09 & 11.4 $\pm$ 0.71 & 2.4 \\
212 & 1.569 & 8.9 $\pm$ 0.15 & 11.6 $\pm$ 0.65 & 3.1 \\
215 & 1.943 & 8.9 $\pm$ 0.88 & 11.3 $\pm$ 0.71 & 2.5 \\
222 & 1.035 & 8.6 $\pm$ 0.14 & 10.9 $\pm$ 0.85 & 3.9 \\
224 & 1.351 & 8.4 $\pm$ 0.09 & 10.9 $\pm$ 0.89 & 3.7 \\
227 & 1.566 & 8.0 $\pm$ 0.2 & 11.0 $\pm$ 0.68 & 2.0 \\
230 & 1.806 & 8.5 $\pm$ 0.14 & 10.5 $\pm$ 0.51 & 4.5 \\
231 & 2.802 & 8.4 $\pm$ 0.05 & 10.6 $\pm$ 0.37 & 3.8 \\
236 & 1.359 & 8.7 $\pm$ 1.02 & 9.7 $\pm$ 0.19 & 2.7 \\
238 & 2.051 & 9.2 $\pm$ 0.08 & 11.2 $\pm$ 0.82 & 3.3 \\
239 & 0.686 & 6.9 $\pm$ 0.24 & 10.8 $\pm$ 0.83 & 1.6 \\
240 & 1.312 & 8.6 $\pm$ 0.2 & 11.0 $\pm$ 0.69 & 4.4 \\
249 & 1.454 & 9.2 $\pm$ 0.04 & 11.2 $\pm$ 0.53 & 2.4 \\
253 & 1.313 & 7.5 $\pm$ 0.39 & 10.8 $\pm$ 0.79 & 4.1 \\
260 & 1.528 & 8.1 $\pm$ 0.21 & 10.9 $\pm$ 0.7 & 3.7 \\
263 & 1.743 & 8.0 $\pm$ 0.46 & 10.6 $\pm$ 0.43 & 1.5 \\
266 & 2.169 & 8.5 $\pm$ 0.14 & 10.7 $\pm$ 0.58 & 4.5 \\
279 & 1.214 & 8.6 $\pm$ 0.16 & 10.5 $\pm$ 0.73 & 3.4 \\
284 & 1.951 & 7.1 $\pm$ 0.08 & 10.7 $\pm$ 0.54 & 1.7 \\
286 & 1.22 & 7.8 $\pm$ 0.08 & 11.1 $\pm$ 0.62 & 3.3 \\
295 & 1.137 & 8.4 $\pm$ 0.19 & 10.9 $\pm$ 0.66 & 2.3 \\
297 & 1.517 & 9.0 $\pm$ 0.93 & 11.4 $\pm$ 1.3 & 2.9 \\
297 & 1.516 & 8.2 $\pm$ 0.93 & 11.4 $\pm$ 0.75 & 2.5 \\
303 & 1.167 & 8.1 $\pm$ 0.18 & 10.8 $\pm$ 0.86 & 3.9 \\
307 & 1.738 & 8.1 $\pm$ 0.41 & 11.1 $\pm$ 0.63 & 1.6 \\
321 & 0.731 & 7.4 $\pm$ 0.27 & 10.3 $\pm$ 0.47 & 0.9 \\
344 & 1.548 & 8.0 $\pm$ 1.04 & 10.0 $\pm$ 0.13 & 1.6 \\
351 & 0.528 & 7.1 $\pm$ 0.49 & 10.4 $\pm$ 1.0 & 0.9 \\
377 & 1.358 & 8.0 $\pm$ 0.28 & 10.8 $\pm$ 1.3 & 4.6 \\
382 & 3.015 & 8.3 $\pm$ 0.11 & 10.5 $\pm$ 0.15 & 1.5 \\
414 & 1.869 & 7.8 $\pm$ 0.16 & 10.5 $\pm$ 0.62 & 3.2 \\
417 & 3.225 & 8.9 $\pm$ 0.14 & 11.3 $\pm$ 0.72 & 4.1 \\
432 & 2.101 & 8.9 $\pm$ 0.2 & 11.4 $\pm$ 0.79 & 2.4 \\
436 & 1.187 & 8.2 $\pm$ 0.11 & 11.2 $\pm$ 0.72 & 4.7 \\
\hline
\end{longtable}

==> yamada.tex <==
\section{Yamada}
%\newcommand{\Rnum}[1]{\setcounter{num}{#1} \Roman{num}}
% \newcommand{\rnum}[1]{\setcounter{num}{#1} \roman{num}}
% \newcounter{num}
% \setcounter{num}{4} 
% \subsection{Search for the low-mass SMBH using the optical variability selection}

We here discuss the possible interpretation of our results in the previous section in terms of coevolution of SMBH and their host galaxies.

In Figure \ref{s-ratio-bin}, we find that the BH to stellar mass ratios show considerably large values for the most massive SMBH with $10^9\leq\MBH/\Ms<10^10$. The red dashed line shows the average value, $\mathrm{log}\ (\MBH/\Mstar)$=$-1.5$, for the 7 objects at $1.5 < z < 3$, which is much larger than the BH-bulge ratio, $\mathrm{log}\ \MBH$/$\Mbulge$=$-2.2$, in the local universe for the same BH mass \citep[e.g.,][]{kormendy2013coevolution}.
The presence of such overmassive BH implies that there is a typical growth path of very massive BHs which is faster than the formation of stars in the associated bulges/spheroids as final products yet to reach the canonical mass ratio in the end. At the higher redshift, $z>4$, \cite{izumi2019subaru} and \cite{pensabene2020alma} found that the BH-dynamical mass ratios also show the similar large value, $\mathrm{log}\ \MBH/\Mdyn\ge-2$.  Our results suggests that such overmassive BH appears not only at the very early universe where the gas cooling efficiency is high but also at the intermediate redshift at $1.5<z<3$.

\citet{croton2006evolution} investigated the evolution of $\MBH-\Mbulge$ relationship in their semi-analytic simulation. They argue that if galaxy mergers are the primary drivers for both BH and bulge growth, one should expect the $\MBH-\Mbulge$ relation to evolve with redshift, with a larger black hole mass associated with a given bulge mass at earlier times relative to the present day. In this model, the growth of bulge mass is due to the disruption of the disks in merging events. This model predicts continuous decrease of BH-bulge mass ratio from $\mathrm{log}\ (\MBH$/$\Mstar)$=$-2.5$ to $-2.7$ (their 'static' model) or from $\mathrm{log}\ (\MBH$/$\Mstar)$=$-2.3$ to $-3$ ('dynamical' model) for the redshift from $z=4$ to 0, depending on the BH mass feeding efficiency. Their model with high BH feeding efficiency predicts as high BH-host mass ratio as observed at $z>4$ but seems not consistent with the similarly high ratio at $1.5<z<3$ as seen in our results.

In the local universe, hosts of the most of the SMBH in this mass range are giant elliptical galaxies. Presence of overmassive BH even at intermediate redshift implies that the growth of stellar component occurs later than their observed epoch. In fact, \citet{mortlock2013redshift} showed that the fraction of the spheroidal galaxies increase from $z=3$ to $z=1$ among the massive galaxies with $\Mstar>10^{10} \Ms$ \citep[see also][]{tasca2014zcosmos}. How these early-type galaxies increase their stellar mass after the formation of their central BH? The two-phase models \citep{oser2010two} with later growth of mass by successive dry mergers can explain the properties of local elliptical galaxies and their plausible progenitors at high-redshift simultaneously. It is, however, puzzling how the very tight $\MBH-\Mbulge$ relation is constructed as their end product as seen in the local universe. Early BH formation should know the later merging mass of halo, which seems inconsistent with the random phase density fluctuation in the early universe.

% \subsection{Redshift evolution of the BH-bulge mass ratio in less massive SMBH}
We also consider the cases for less massive SMBHs with $10^7\leq \MBH/\Ms<10^9$ whose BH-stellar mass ratio do not appear to evolve significantly over the observed redshift range for the given BH mass.
The difference in the mass ratio between BH with $10^8\leq\MBH/\Ms<10^9$ and those with $10^7\leq\MBH/\Ms<10^8$ can be explained by the contribution of disk components in their stellar mass, as the host of BH with $10^8\leq\MBH/\Ms<10^9$, or with $\Mstar \sim 10^{11-12}M_\odot$, are typically early-type galaxies while the less massive BH with $10^7\leq\MBH/\Ms<10^8$ tend to reside also in disk galaxies.

The nearly constant BH to stellar mass ratio over the redshift range may indicate that the BH and bulges always co-evolve in their formation history if there is no contribution of the disk components. In this case, however, the BH to stellar mass ratio should also be similar for the different BH mass range over their growth, which is not seen in our results. It is also not consistent that the BH to stellar mass ratio for a given BH mass range at the intermediate redshift is similar with those observed at the local universe in the same BH mass range.

Alternatively, the observed AGN at the intermediate redshift have already acquired their present-day structure in terms of the BH, bulge, and disk components. In other words, what we observe as AGN with $7\leq\MBH/\Ms<9$ at $0.5<z<3$ are nearly the end products of their BH and galaxy formation. This contrasts with the recent discovery of the overmassive BH in this mass range at the higher redshift, $4<z<7$ \citep[e.g.,][]{harikane2023jwst,maiolino2023jades}. We speculate that BH appears in overmassive with their bulge progenitors in such high redshift objects, as their more massive counterparts with $\MBH/\Ms>10^9$.

Pacucci et al. (2024) show the interpretation of the overmassive BH with the assumption that black hole mass growth is regulated by the quasar's output, and the stellar mass growth is also quenched by it. This process works at high redshift when the host galaxies are physically small, and the accretion duty cycle is high, but a runaway process brings the originally overmassive system towards the local BH to stellar mass relation once the condition of suppressing star-formation is broken. This can explain at least the behavior of less massive BH objects in our sample.

==> zbhmass_latex_with_kimura.tex <==
\begin{longtable}{|c|c|c|c|c|c|c|c|c|c|}
\hline
\hline
varAGN ID & R.A.(J2000) & Dec.(J2000) & $i$-band & Redshift & $FWHM$ & $\MBH$ & $\Lbol$ & S/N & line \\
\hline
  & [deg] & [deg] & [mag] &  & [$10^3\ \mathrm{km\ s^{-1}}$] & [$\Ms$] & [$\mathrm{erg\ s^{-1}}$] &  &  \\
\hline
(1) & (2) & (3) & (4) & (5) & (6) & (7) & (8) & (9) & (10) \\
\hline
\endhead\hline\endfoot
1 & 150.74386 & 2.20245 & 22.71 & 1.618 & 6.4 $\pm$ 1.17 & 8.6 $\pm$ 1.08 & 45.3 & 6.63 & 2 \\
2 & 150.73557 & 2.19957 & 20.36 & 3.497 & 5.6 $\pm$ 0.03 & 8.8 $\pm$ 0.16 & 45.9 & 4.76 & 2 \\
7 & 150.78838 & 2.34399 & 19.82 & 1.964 & 4.6 $\pm$ 0.0 & 8.5 $\pm$ 0.07 & 45.8 & 7.46 & 2 \\
8 & 150.71511 & 2.48483 & 19.2 & 2.003 & 4.4 $\pm$ 0.0 & 8.5 $\pm$ 0.04 & 45.8 & 8.95 & 2 \\
12 & 150.65294 & 1.99685 & 19.52 & 1.518 & 3.0 $\pm$ 0.03 & 7.9 $\pm$ 0.19 & 45.1 & 8.03 & 1 \\
15 & 150.61224 & 1.99442 & 21.4 & 1.609 & 3.1 $\pm$ 0.16 & 7.8 $\pm$ 0.4 & 45.0 & 6.42 & 1 \\
16 & 150.57489 & 1.97677 & 20.98 & 1.541 & 4.9 $\pm$ 0.01 & 8.5 $\pm$ 0.08 & 45.5 & 11.98 & 1 \\
17 & 150.55903 & 2.10576 & 22.61 & 2.33 & 4.9 $\pm$ 0.14 & 8.8 $\pm$ 0.38 & 46.1 & 11.52 & 1 \\
19 & 150.70416 & 2.29746 & 21.59 & 2.74 & 3.5 $\pm$ 0.05 & 8.2 $\pm$ 0.22 & 45.5 & 99.99 & 2 \\
20 & 150.70801 & 2.29233 & 21.09 & 1.099 & 6.1 $\pm$ 0.0 & 8.5 $\pm$ 0.04 & 45.3 & 12.33 & 1 \\
22 & 150.58112 & 2.22107 & 21.92 & 2.023 & 6.3 $\pm$ 0.3 & 8.6 $\pm$ 0.55 & 45.3 & 5.9 & 1 \\
23 & 150.53187 & 2.18892 & 21.58 & 0.827 & 1.5 $\pm$ 0.02 & 7.0 $\pm$ 0.19 & 44.5 & 8.74 & 1 \\
24 & 150.6097 & 2.32311 & 20.44 & 1.295 & 2.4 $\pm$ 0.28 & 8.0 $\pm$ 0.53 & 45.9 & 15.3 & 1 \\
26 & 150.6302 & 2.45454 & 20.2 & 0.817 & 4.9 $\pm$ 0.13 & 8.0 $\pm$ 0.38 & 44.5 & 8.63 & 1 \\
27 & 150.55556 & 2.36917 & 23.29 & 1.64 & 4.2 $\pm$ 0.32 & 7.9 $\pm$ 0.59 & 44.7 & 3.33 & 2 \\
28 & 150.59971 & 2.39823 & 20.77 & 2.836 & 2.4 $\pm$ 0.03 & 7.7 $\pm$ 0.18 & 45.3 & 3.9 & 2 \\
28 & 150.59971 & 2.39823 & 20.77 & 2.83 & 8.0 $\pm$ 0.33 & 8.8 $\pm$ 0.57 & 45.3 & 3.9 & 2 \\
30 & 150.61728 & 2.48275 & 22.59 & 2.733 & 7.9 $\pm$ 0.26 & 8.9 $\pm$ 0.51 & 45.5 & 4.25 & 2 \\
33 & 150.68315 & 2.57464 & 19.16 & 0.376 & 3.0 $\pm$ 0.01 & 7.4 $\pm$ 0.12 & 44.6 & 20.83 & 3 \\
34 & 150.63388 & 2.59371 & 19.13 & 0.657 & 2.8 $\pm$ 0.0 & 7.8 $\pm$ 0.05 & 45.2 & 21.78 & 1 \\
36 & 150.70554 & 2.6296 & 19.97 & 2.122 & 3.0 $\pm$ 0.02 & 8.3 $\pm$ 0.15 & 45.9 & 10.55 & 1 \\
37 & 150.63539 & 2.64991 & 21.04 & 1.223 & 5.2 $\pm$ 0.01 & 8.1 $\pm$ 0.15 & 44.7 & 5.64 & 1 \\
39 & 150.53932 & 2.54206 & 21.94 & 1.716 & 1.9 $\pm$ 0.38 & 7.4 $\pm$ 0.62 & 45.0 & 5.26 & 1 \\
43 & 150.55489 & 2.64105 & 21.58 & 1.142 & 6.5 $\pm$ 0.01 & 8.6 $\pm$ 0.09 & 45.2 & 12.06 & 1 \\
44 & 150.59735 & 2.61793 & 21.27 & 1.447 & 5.0 $\pm$ 0.01 & 8.3 $\pm$ 0.11 & 45.1 & 7.63 & 1 \\
46 & 150.44749 & 1.69569 & 22.04 & 2.16 & 2.3 $\pm$ 0.65 & 7.3 $\pm$ 0.8 & 44.4 & 99.99 & 1 \\
47 & 150.37654 & 1.7179 & 20.06 & 1.571 & 3.8 $\pm$ 0.09 & 8.2 $\pm$ 0.3 & 45.5 & 8.86 & 1 \\
51 & 150.49127 & 1.91029 & 21.95 & 2.234 & 2.0 $\pm$ 0.1 & 7.4 $\pm$ 0.36 & 44.8 & 3.31 & 1 \\
58 & 150.35942 & 1.93644 & 22.48 & 2.367 & 7.5 $\pm$ 1.47 & 8.6 $\pm$ 1.21 & 45.1 & 99.99 & 2 \\
60 & 150.43102 & 1.93527 & 21.47 & 2.171 & 6.3 $\pm$ 0.47 & 8.8 $\pm$ 0.69 & 45.6 & 9.02 & 1 \\
61 & 150.40096 & 1.91198 & 21.06 & 2.28 & 7.6 $\pm$ 0.08 & 9.1 $\pm$ 0.28 & 46.0 & 11.15 & 2 \\
63 & 150.44602 & 2.04351 & 20.82 & 1.171 & 8.1 $\pm$ 0.0 & 8.9 $\pm$ 0.06 & 45.4 & 13.07 & 1 \\
64 & 150.44368 & 2.0491 & 20.11 & 0.669 & 2.1 $\pm$ 0.01 & 7.5 $\pm$ 0.09 & 45.1 & 17.88 & 1 \\
66 & 150.42256 & 2.01415 & 21.79 & 2.283 & 4.5 $\pm$ 0.08 & 8.3 $\pm$ 0.28 & 45.3 & 6.12 & 1 \\
68 & 150.41834 & 2.08515 & 20.08 & 0.424 & 2.5 $\pm$ 0.07 & 7.0 $\pm$ 0.32 & 44.4 & 13.49 & 3 \\
70 & 150.45184 & 2.14481 & 20.64 & 1.298 & 1.7 $\pm$ 0.01 & 7.1 $\pm$ 0.17 & 44.7 & 5.63 & 1 \\
71 & 150.48437 & 2.16202 & 21.84 & 1.639 & 8.4 $\pm$ 0.01 & 8.9 $\pm$ 0.1 & 45.4 & 11.07 & 1 \\
73 & 150.4496 & 2.24643 & 20.67 & 0.882 & 3.0 $\pm$ 0.01 & 7.8 $\pm$ 0.11 & 45.1 & 11.88 & 1 \\
75 & 150.51907 & 2.32098 & 22.24 & 1.836 & 5.6 $\pm$ 0.02 & 8.6 $\pm$ 0.13 & 45.6 & 11.6 & 1 \\
77 & 150.36472 & 2.1438 & 23.24 & 3.328 & 2.7 $\pm$ 0.03 & 8.1 $\pm$ 0.18 & 45.9 & 4.43 & 2 \\
78 & 150.37824 & 2.19636 & 22.49 & 1.512 & 5.2 $\pm$ 0.02 & 8.5 $\pm$ 0.15 & 45.4 & 9.87 & 1 \\
79 & 150.34592 & 2.14752 & 20.74 & 1.256 & 2.9 $\pm$ 0.01 & 7.8 $\pm$ 0.11 & 45.1 & 99.99 & 1 \\
81 & 150.42223 & 2.17535 & 20.94 & 0.979 & 4.0 $\pm$ 0.01 & 8.2 $\pm$ 0.1 & 45.3 & 14.05 & 1 \\
83 & 150.37463 & 2.3102 & 23.05 & 2.155 & 8.1 $\pm$ 0.6 & 8.8 $\pm$ 0.77 & 45.3 & 5.28 & 2 \\
85 & 150.43817 & 2.41581 & 20.49 & 2.02 & 9.7 $\pm$ 0.01 & 8.9 $\pm$ 0.12 & 45.2 & 5.58 & 2 \\
87 & 150.49565 & 2.41256 & 21.62 & 1.369 & 5.7 $\pm$ 0.0 & 8.4 $\pm$ 0.07 & 45.1 & 9.27 & 1 \\
89 & 150.51157 & 2.40961 & 20.99 & 0.986 & 6.0 $\pm$ 0.04 & 8.4 $\pm$ 0.21 & 45.0 & 11.48 & 1 \\
91 & 150.49911 & 2.44491 & 19.03 & 2.03 & 4.6 $\pm$ 0.01 & 9.1 $\pm$ 0.11 & 46.9 & 21.1 & 1 \\
92 & 150.35363 & 2.34216 & 20.36 & 1.714 & 1.9 $\pm$ 0.42 & 7.8 $\pm$ 0.65 & 45.8 & 11.12 & 4 \\
93 & 150.40669 & 2.36546 & 21.8 & 2.037 & 2.8 $\pm$ 0.05 & 7.7 $\pm$ 0.23 & 45.1 & 99.99 & 2 \\
95 & 150.4536 & 2.5279 & 21.03 & 1.931 & 2.6 $\pm$ 0.05 & 7.8 $\pm$ 0.22 & 45.2 & 4.76 & 1 \\
96 & 150.45666 & 2.64811 & 20.36 & 2.05 & 4.5 $\pm$ 0.02 & 8.5 $\pm$ 0.15 & 45.7 & 9.11 & 1 \\
97 & 150.49762 & 2.65989 & 19.94 & 0.854 & 11.6 $\pm$ 0.0 & 9.1 $\pm$ 0.03 & 45.2 & 15.86 & 1 \\
99 & 150.38283 & 2.55977 & 22.94 & 2.068 & 7.1 $\pm$ 0.26 & 8.5 $\pm$ 0.52 & 45.0 & 3.98 & 2 \\
100 & 150.41596 & 2.52574 & 22.27 & 1.444 & 2.3 $\pm$ 0.01 & 7.5 $\pm$ 0.13 & 44.9 & 5.71 & 1 \\
101 & 150.35143 & 2.67822 & 21.15 & 2.754 & 8.0 $\pm$ 0.01 & 9.2 $\pm$ 0.1 & 46.1 & 8.86 & 2 \\
102 & 150.49077 & 2.77544 & 20.24 & 1.434 & 8.8 $\pm$ 0.01 & 9.4 $\pm$ 0.08 & 46.3 & 22.43 & 1 \\
105 & 150.38285 & 2.72363 & 22.35 & 2.053 & 8.6 $\pm$ 0.58 & 8.8 $\pm$ 0.76 & 45.3 & 6.24 & 2 \\
109 & 150.31993 & 1.68158 & 19.78 & 2.055 & 4.4 $\pm$ 0.01 & 8.6 $\pm$ 0.1 & 46.0 & 8.88 & 2 \\
113 & 150.30622 & 1.87518 & 23.31 & 1.759 & 4.1 $\pm$ 0.75 & 8.1 $\pm$ 0.86 & 45.2 & 99.99 & 2 \\
115 & 150.30889 & 1.91231 & 21.57 & 1.525 & 9.0 $\pm$ 0.9 & 9.1 $\pm$ 0.95 & 45.8 & 13.16 & 1 \\
119 & 150.24519 & 1.90011 & 20.01 & 1.56 & 2.6 $\pm$ 0.11 & 8.2 $\pm$ 0.33 & 46.0 & 15.43 & 1 \\
120 & 150.20823 & 1.87538 & 20.52 & 1.147 & 8.2 $\pm$ 0.03 & 8.6 $\pm$ 0.2 & 44.9 & 6.85 & 1 \\
121 & 150.24309 & 1.86912 & 20.58 & 2.027 & 3.5 $\pm$ 0.03 & 8.1 $\pm$ 0.18 & 45.4 & 6.33 & 1 \\
122 & 150.16179 & 1.87796 & 21.98 & 1.444 & 2.9 $\pm$ 0.0 & 7.9 $\pm$ 0.06 & 45.2 & 8.41 & 1 \\
124 & 150.25342 & 1.99661 & 21.93 & 1.171 & 8.2 $\pm$ 0.01 & 8.7 $\pm$ 0.11 & 45.0 & 7.79 & 1 \\
125 & 150.31186 & 1.97795 & 21.72 & 2.351 & 6.8 $\pm$ 0.24 & 8.8 $\pm$ 0.49 & 45.6 & 6.47 & 1 \\
126 & 150.28566 & 2.01459 & 21.2 & 2.654 & 5.6 $\pm$ 0.03 & 8.8 $\pm$ 0.19 & 46.0 & 7.33 & 2 \\
128 & 150.33439 & 2.06147 & 20.17 & 0.904 & 3.5 $\pm$ 0.02 & 7.8 $\pm$ 0.16 & 44.7 & 7.91 & 1 \\
129 & 150.30691 & 2.05384 & 23.6 & 2.005 & 6.2 $\pm$ 1.12 & 8.4 $\pm$ 1.06 & 45.0 & 4.04 & 2 \\
130 & 150.21637 & 1.98874 & 21.34 & 2.23 & 4.5 $\pm$ 0.14 & 8.6 $\pm$ 0.37 & 46.0 & 10.27 & 1 \\
131 & 150.18074 & 2.07598 & 22.87 & 2.994 & 5.8 $\pm$ 0.26 & 9.0 $\pm$ 0.51 & 46.3 & 99.99 & 2 \\
132 & 150.27217 & 2.23009 & 21.02 & 2.611 & 15.2 $\pm$ 0.06 & 9.9 $\pm$ 0.24 & 46.3 & 10.95 & 2 \\
133 & 150.30261 & 2.16108 & 20.23 & 1.817 & 4.5 $\pm$ 0.0 & 8.2 $\pm$ 0.08 & 45.1 & 5.05 & 1 \\
134 & 150.31652 & 2.24678 & 21.62 & 2.483 & 3.3 $\pm$ 0.12 & 8.0 $\pm$ 0.34 & 45.4 & 5.18 & 2 \\
136 & 150.15843 & 2.13957 & 20.14 & 1.829 & 5.7 $\pm$ 0.05 & 8.5 $\pm$ 0.24 & 45.3 & 6.12 & 1 \\
138 & 150.21469 & 2.20427 & 20.7 & 1.841 & 3.1 $\pm$ 0.01 & 8.2 $\pm$ 0.08 & 45.7 & 10.46 & 1 \\
139 & 150.19979 & 2.19085 & 20.92 & 1.515 & 8.5 $\pm$ 0.01 & 8.8 $\pm$ 0.08 & 45.2 & 7.45 & 1 \\
140 & 150.23628 & 2.28913 & 21.36 & 2.083 & 7.1 $\pm$ 0.13 & 8.4 $\pm$ 0.38 & 44.9 & 3.53 & 2 \\
142 & 150.25271 & 2.48638 & 21.15 & 2.04 & 7.3 $\pm$ 0.31 & 8.6 $\pm$ 0.56 & 45.1 & 5.22 & 1 \\
143 & 150.30809 & 2.43003 & 20.25 & 0.373 & 4.0 $\pm$ 0.04 & 7.3 $\pm$ 0.39 & 44.2 & 12.54 & 3 \\
144 & 150.29976 & 2.50687 & 21.03 & 1.503 & 1.8 $\pm$ 0.32 & 7.3 $\pm$ 0.57 & 45.1 & 8.07 & 4 \\
147 & 150.23182 & 2.36399 & 20.68 & 1.936 & 4.9 $\pm$ 0.01 & 8.5 $\pm$ 0.12 & 45.5 & 7.46 & 1 \\
149 & 150.24463 & 2.43227 & 20.63 & 0.696 & 3.3 $\pm$ 0.06 & 7.4 $\pm$ 0.28 & 44.6 & 11.71 & 3 \\
150 & 150.20902 & 2.43846 & 21.0 & 3.715 & 8.5 $\pm$ 0.01 & 9.3 $\pm$ 0.11 & 46.3 & 99.99 & 2 \\
151 & 150.20887 & 2.48189 & 19.71 & 3.333 & 4.9 $\pm$ 0.0 & 8.6 $\pm$ 0.05 & 45.7 & 4.44 & 2 \\
152 & 150.29252 & 2.54507 & 21.48 & 2.653 & 6.0 $\pm$ 0.02 & 8.9 $\pm$ 0.13 & 46.1 & 9.45 & 2 \\
153 & 150.32383 & 2.55258 & 22.83 & 1.002 & 1.8 $\pm$ 0.12 & 7.1 $\pm$ 0.36 & 44.9 & 9.99 & 4 \\
154 & 150.31791 & 2.60207 & 20.86 & 0.958 & 3.9 $\pm$ 0.18 & 8.2 $\pm$ 0.42 & 45.4 & 13.66 & 1 \\
155 & 150.33446 & 2.56146 & 19.86 & 1.836 & 3.2 $\pm$ 0.01 & 8.0 $\pm$ 0.12 & 45.3 & 6.98 & 1 \\
158 & 150.2978 & 2.67347 & 21.83 & 1.603 & 12.1 $\pm$ 1.39 & 8.9 $\pm$ 1.18 & 44.8 & 5.37 & 1 \\
160 & 150.16384 & 2.59765 & 21.91 & 1.589 & 4.7 $\pm$ 0.05 & 8.2 $\pm$ 0.22 & 45.0 & 5.55 & 1 \\
162 & 150.23083 & 2.57815 & 19.58 & 1.402 & 6.9 $\pm$ 0.01 & 8.9 $\pm$ 0.09 & 45.7 & 13.82 & 1 \\
165 & 150.29771 & 2.73879 & 23.22 & 1.954 & 3.8 $\pm$ 0.06 & 8.0 $\pm$ 0.24 & 45.1 & 5.47 & 2 \\
166 & 150.33854 & 2.7767 & 22.94 & 2.126 & 4.5 $\pm$ 0.44 & 8.4 $\pm$ 0.66 & 45.6 & 9.26 & 2 \\
168 & 150.25135 & 2.73714 & 20.76 & 2.167 & 4.7 $\pm$ 0.05 & 8.5 $\pm$ 0.22 & 45.6 & 7.5 & 1 \\
169 & 150.16706 & 2.76891 & 21.92 & 2.388 & 6.3 $\pm$ 0.39 & 8.4 $\pm$ 0.63 & 45.1 & 3.49 & 2 \\
170 & 150.05185 & 1.68279 & 20.17 & 2.276 & 6.1 $\pm$ 0.0 & 8.8 $\pm$ 0.06 & 45.8 & 8.92 & 2 \\
171 & 149.99161 & 1.72432 & 20.21 & 1.625 & 4.0 $\pm$ 0.11 & 8.2 $\pm$ 0.33 & 45.3 & 7.67 & 1 \\
172 & 150.13175 & 1.79944 & 20.84 & 1.679 & 8.6 $\pm$ 0.02 & 9.2 $\pm$ 0.13 & 45.9 & 12.24 & 1 \\
173 & 150.12456 & 1.80983 & 22.71 & 1.358 & 2.1 $\pm$ 0.32 & 7.6 $\pm$ 0.56 & 45.1 & 99.99 & 1 \\
174 & 150.10166 & 1.84837 & 19.81 & 1.666 & 2.2 $\pm$ 0.01 & 7.6 $\pm$ 0.12 & 45.3 & 7.5 & 4 \\
176 & 150.08145 & 1.90601 & 23.08 & 1.817 & 4.5 $\pm$ 0.53 & 7.7 $\pm$ 0.85 & 44.2 & 3.68 & 2 \\
179 & 149.98874 & 1.93244 & 22.58 & 2.405 & 5.0 $\pm$ 0.23 & 8.2 $\pm$ 0.48 & 45.0 & 3.51 & 2 \\
183 & 149.99527 & 2.00665 & 21.97 & 1.033 & 1.5 $\pm$ 0.26 & 6.9 $\pm$ 0.52 & 44.8 & 7.3 & 4 \\
184 & 150.0044 & 2.03891 & 21.55 & 3.499 & 4.2 $\pm$ 0.01 & 8.3 $\pm$ 0.08 & 45.5 & 3.66 & 2 \\
185 & 150.05894 & 2.01516 & 19.63 & 2.498 & 3.5 $\pm$ 0.0 & 8.5 $\pm$ 0.06 & 46.1 & 9.29 & 2 \\
186 & 149.99176 & 2.13195 & 22.85 & 2.131 & 5.3 $\pm$ 0.69 & 8.5 $\pm$ 0.83 & 45.3 & 4.36 & 1 \\
190 & 150.13803 & 2.29165 & 17.56 & 0.185 & 0.9 $\pm$ 0.0 & 5.8 $\pm$ 0.67 & 43.8 & 15.68 & 4 \\
195 & 149.99391 & 2.30143 & 19.89 & 1.796 & 6.1 $\pm$ 0.02 & 8.8 $\pm$ 0.14 & 45.9 & 11.83 & 1 \\
196 & 150.00447 & 2.23711 & 21.61 & 1.406 & 3.3 $\pm$ 0.0 & 8.1 $\pm$ 0.05 & 45.5 & 10.82 & 1 \\
197 & 150.06456 & 2.32902 & 21.85 & 2.45 & 6.3 $\pm$ 0.06 & 8.6 $\pm$ 0.26 & 45.3 & 4.05 & 1 \\
198 & 150.09156 & 2.39905 & 21.75 & 2.47 & 3.7 $\pm$ 0.09 & 8.5 $\pm$ 0.3 & 46.0 & 8.97 & 2 \\
199 & 150.12369 & 2.35825 & 20.03 & 0.728 & 1.8 $\pm$ 0.16 & 7.1 $\pm$ 0.41 & 44.9 & 12.43 & 3 \\
201 & 150.00423 & 2.38915 & 23.28 & 1.846 & 1.9 $\pm$ 0.04 & 7.4 $\pm$ 0.22 & 45.0 & 4.7 & 1 \\
203 & 150.05873 & 2.47739 & 20.62 & 1.258 & 5.2 $\pm$ 0.01 & 8.4 $\pm$ 0.09 & 45.2 & 9.94 & 1 \\
207 & 150.10447 & 2.69123 & 21.21 & 1.881 & 2.8 $\pm$ 0.07 & 8.1 $\pm$ 0.26 & 45.7 & 11.3 & 1 \\
209 & 150.12689 & 2.62654 & 21.68 & 1.839 & 2.6 $\pm$ 0.04 & 8.0 $\pm$ 0.2 & 45.7 & 10.89 & 1 \\
211 & 150.04526 & 2.68849 & 21.78 & 1.438 & 2.5 $\pm$ 0.07 & 7.8 $\pm$ 0.27 & 45.4 & 12.39 & 1 \\
212 & 150.04251 & 2.62916 & 20.44 & 1.569 & 7.5 $\pm$ 0.02 & 8.9 $\pm$ 0.15 & 45.7 & 11.05 & 1 \\
214 & 150.06065 & 2.64796 & 20.87 & 0.437 & 3.5 $\pm$ 0.02 & 7.0 $\pm$ 1.2 & 44.0 & 6.13 & 3 \\
215 & 150.03066 & 2.67873 & 21.46 & 1.943 & 10.0 $\pm$ 0.77 & 8.9 $\pm$ 0.88 & 45.2 & 5.57 & 1 \\
222 & 149.81688 & 1.84673 & 20.76 & 1.035 & 8.3 $\pm$ 0.02 & 8.6 $\pm$ 0.14 & 44.9 & 10.64 & 1 \\
224 & 149.82193 & 1.83866 & 20.93 & 1.351 & 4.8 $\pm$ 0.01 & 8.4 $\pm$ 0.09 & 45.3 & 10.84 & 1 \\
227 & 149.79179 & 1.87287 & 22.21 & 1.566 & 4.2 $\pm$ 0.03 & 8.0 $\pm$ 0.2 & 44.8 & 5.33 & 1 \\
228 & 149.92256 & 1.97922 & 22.24 & 2.508 & 3.6 $\pm$ 0.11 & 8.2 $\pm$ 0.32 & 45.5 & 5.58 & 2 \\
230 & 149.95773 & 2.0031 & 20.82 & 1.806 & 5.6 $\pm$ 0.02 & 8.5 $\pm$ 0.14 & 45.3 & 4.96 & 1 \\
231 & 149.90955 & 2.08058 & 20.35 & 2.802 & 4.3 $\pm$ 0.0 & 8.4 $\pm$ 0.05 & 45.6 & 5.4 & 2 \\
232 & 149.89793 & 2.09392 & 21.49 & 1.921 & 3.0 $\pm$ 0.05 & 8.1 $\pm$ 0.23 & 45.6 & 8.24 & 1 \\
235 & 149.8951 & 2.04721 & 21.78 & 2.198 & 4.3 $\pm$ 0.01 & 8.3 $\pm$ 0.08 & 45.3 & 5.32 & 1 \\
236 & 149.81421 & 2.01633 & 22.48 & 1.359 & 8.3 $\pm$ 1.03 & 8.8 $\pm$ 1.02 & 45.3 & 9.16 & 1 \\
238 & 149.82269 & 2.08965 & 21.87 & 2.051 & 10.4 $\pm$ 0.01 & 9.2 $\pm$ 0.08 & 45.6 & 7.64 & 1 \\
239 & 149.91244 & 2.20032 & 20.3 & 0.686 & 1.5 $\pm$ 0.03 & 6.9 $\pm$ 0.24 & 44.5 & 7.85 & 1 \\
240 & 149.89483 & 2.17443 & 21.55 & 1.312 & 6.7 $\pm$ 0.04 & 8.6 $\pm$ 0.2 & 45.1 & 7.15 & 1 \\
241 & 149.8954 & 2.23947 & 20.7 & 1.729 & 3.5 $\pm$ 0.11 & 7.9 $\pm$ 0.35 & 45.0 & 3.86 & 1 \\
242 & 149.7819 & 2.13906 & 18.54 & 0.354 & 6.0 $\pm$ 0.11 & 8.1 $\pm$ 0.35 & 44.3 & 16.43 & 1 \\
244 & 149.78977 & 2.3212 & 20.07 & 0.378 & 1.9 $\pm$ 0.02 & 6.8 $\pm$ 0.27 & 44.4 & 12.15 & 4 \\
249 & 149.91977 & 2.32742 & 20.27 & 1.454 & 7.3 $\pm$ 0.0 & 9.2 $\pm$ 0.04 & 46.3 & 19.79 & 1 \\
251 & 149.91694 & 2.38518 & 19.78 & 1.131 & 3.3 $\pm$ 0.0 & 8.0 $\pm$ 0.04 & 45.3 & 12.09 & 1 \\
252 & 149.88334 & 2.34673 & 21.46 & 1.021 & 3.0 $\pm$ 0.1 & 7.6 $\pm$ 0.34 & 44.7 & 6.85 & 1 \\
253 & 149.88102 & 2.45083 & 21.51 & 1.313 & 2.8 $\pm$ 0.01 & 7.5 $\pm$ 0.39 & 44.5 & 3.46 & 1 \\
256 & 149.95563 & 2.50204 & 22.38 & 1.458 & 8.1 $\pm$ 0.0 & 8.9 $\pm$ 0.05 & 45.5 & 10.74 & 1 \\
258 & 149.81293 & 2.34546 & 21.54 & 1.812 & 4.7 $\pm$ 0.09 & 8.1 $\pm$ 0.33 & 44.9 & 3.75 & 1 \\
260 & 149.87071 & 2.41727 & 21.93 & 1.528 & 5.1 $\pm$ 0.02 & 8.1 $\pm$ 0.21 & 44.8 & 4.52 & 1 \\
262 & 149.86806 & 2.33069 & 20.55 & 1.478 & 4.3 $\pm$ 0.0 & 8.2 $\pm$ 0.04 & 45.2 & 8.32 & 1 \\
263 & 149.87184 & 2.34286 & 21.55 & 1.743 & 3.7 $\pm$ 0.2 & 8.0 $\pm$ 0.46 & 45.0 & 4.84 & 1 \\
265 & 149.91067 & 2.55465 & 19.96 & 0.753 & 6.4 $\pm$ 0.25 & 7.9 $\pm$ 1.39 & 44.0 & 3.41 & 1 \\
266 & 149.87591 & 2.69026 & 21.39 & 2.169 & 4.8 $\pm$ 0.02 & 8.5 $\pm$ 0.14 & 45.7 & 9.68 & 2 \\
269 & 149.9254 & 2.68423 & 20.28 & 1.779 & 3.6 $\pm$ 0.01 & 8.0 $\pm$ 0.13 & 45.1 & 4.35 & 2 \\
270 & 149.78564 & 2.55479 & 22.32 & 1.798 & 4.6 $\pm$ 0.41 & 8.3 $\pm$ 0.64 & 45.3 & 7.65 & 1 \\
272 & 149.81144 & 2.55798 & 23.03 & 2.152 & 4.5 $\pm$ 0.52 & 8.1 $\pm$ 0.72 & 45.0 & 4.62 & 2 \\
273 & 149.86032 & 2.54475 & 22.77 & 1.596 & 8.5 $\pm$ 0.02 & 8.9 $\pm$ 0.16 & 45.4 & 9.24 & 1 \\
274 & 149.808 & 2.64568 & 21.19 & 2.082 & 7.7 $\pm$ 0.05 & 9.0 $\pm$ 0.23 & 45.8 & 9.9 & 1 \\
279 & 149.68747 & 1.81266 & 22.58 & 1.214 & 7.7 $\pm$ 0.02 & 8.6 $\pm$ 0.16 & 45.0 & 8.36 & 1 \\
280 & 149.64996 & 1.86587 & 19.48 & 2.935 & 4.3 $\pm$ 0.13 & 8.4 $\pm$ 0.36 & 45.6 & 5.16 & 2 \\
281 & 149.67418 & 1.88837 & 19.97 & 1.77 & 8.8 $\pm$ 0.07 & 9.3 $\pm$ 0.27 & 46.2 & 14.51 & 1 \\
282 & 149.71561 & 2.01652 & 23.08 & 2.686 & 2.1 $\pm$ 0.0 & 7.7 $\pm$ 0.07 & 45.5 & 4.86 & 2 \\
283 & 149.74451 & 2.02752 & 19.39 & 2.448 & 8.9 $\pm$ 0.03 & 9.5 $\pm$ 0.16 & 46.6 & 13.33 & 2 \\
284 & 149.75359 & 2.12563 & 22.36 & 1.951 & 1.8 $\pm$ 0.01 & 7.1 $\pm$ 0.08 & 44.4 & 99.99 & 1 \\
286 & 149.66361 & 2.08522 & 20.18 & 1.22 & 2.7 $\pm$ 0.01 & 7.8 $\pm$ 0.08 & 45.1 & 10.56 & 1 \\
288 & 149.73896 & 2.22069 & 20.37 & 1.024 & 9.8 $\pm$ 0.02 & 9.7 $\pm$ 0.14 & 46.8 & 31.53 & 1 \\
289 & 149.71125 & 2.14515 & 20.31 & 1.538 & 8.9 $\pm$ 0.45 & 8.7 $\pm$ 0.67 & 44.9 & 99.99 & 1 \\
293 & 149.6668 & 2.28643 & 21.02 & 1.028 & 5.3 $\pm$ 0.07 & 8.3 $\pm$ 0.27 & 45.0 & 11.03 & 1 \\
295 & 149.76348 & 2.33414 & 20.99 & 1.137 & 6.8 $\pm$ 0.02 & 8.4 $\pm$ 0.19 & 44.7 & 6.31 & 1 \\
297 & 149.69877 & 2.44124 & 21.23 & 1.516 & 3.4 $\pm$ 0.86 & 8.2 $\pm$ 0.93 & 45.7 & 8.92 & 4 \\
298 & 149.70583 & 2.4198 & 20.39 & 1.122 & 12.2 $\pm$ 0.0 & 9.6 $\pm$ 0.05 & 46.1 & 22.99 & 1 \\
299 & 149.73852 & 2.43387 & 21.52 & 2.097 & 2.8 $\pm$ 0.02 & 7.7 $\pm$ 0.23 & 44.9 & 3.1 & 1 \\
300 & 149.77692 & 2.44428 & 22.41 & 4.164 & 6.7 $\pm$ 0.25 & 8.9 $\pm$ 0.5 & 45.7 & 99.99 & 2 \\
303 & 149.62804 & 2.4595 & 22.16 & 1.167 & 5.2 $\pm$ 0.02 & 8.1 $\pm$ 0.18 & 44.7 & 6.93 & 1 \\
304 & 149.61116 & 2.47171 & 20.59 & 0.693 & 0.7 $\pm$ 0.06 & 6.3 $\pm$ 0.25 & 44.9 & 13.87 & 3 \\
305 & 149.70361 & 2.5781 & 20.48 & 1.545 & 5.6 $\pm$ 0.02 & 8.6 $\pm$ 0.15 & 45.6 & 12.2 & 1 \\
307 & 149.72134 & 2.54001 & 21.57 & 1.738 & 4.6 $\pm$ 0.16 & 8.2 $\pm$ 0.4 & 45.1 & 4.95 & 1 \\
312 & 149.58664 & 2.03712 & 20.48 & 1.85 & 5.6 $\pm$ 0.0 & 8.9 $\pm$ 0.05 & 46.2 & 13.63 & 1 \\
313 & 149.57351 & 2.02367 & 21.52 & 2.808 & 1.0 $\pm$ 0.05 & 7.1 $\pm$ 0.23 & 45.5 & 5.32 & 2 \\
315 & 149.56469 & 1.9779 & 20.97 & 1.688 & 4.3 $\pm$ 0.02 & 8.5 $\pm$ 0.13 & 45.9 & 10.79 & 1 \\
318 & 149.50675 & 2.07472 & 22.34 & 1.226 & 6.8 $\pm$ 0.02 & 8.6 $\pm$ 0.14 & 45.2 & 7.81 & 1 \\
321 & 149.5731 & 2.32739 & 21.06 & 0.731 & 3.6 $\pm$ 0.04 & 7.4 $\pm$ 0.27 & 44.5 & 10.44 & 3 \\
327 & 150.42196 & 2.38551 & 23.34 & 1.516 & 3.1 $\pm$ 1.67 & 7.9 $\pm$ 1.29 & 45.3 & 8.07 & 4 \\
329 & 150.34122 & 1.76125 & 23.72 & 2.93 & 4.4 $\pm$ 0.09 & 8.0 $\pm$ 0.3 & 44.8 & 99.99 & 2 \\
344 & 149.79629 & 2.55944 & 22.41 & 1.548 & 4.9 $\pm$ 1.07 & 8.2 $\pm$ 1.04 & 45.0 & 5.44 & 2 \\
351 & 150.32723 & 1.9286 & 20.07 & 0.528 & 3.1 $\pm$ 0.0 & 7.1 $\pm$ 0.49 & 44.2 & 7.68 & 3 \\
369 & 150.34772 & 2.39099 & 22.41 & 1.847 & 6.9 $\pm$ 0.02 & 8.7 $\pm$ 0.16 & 45.4 & 6.52 & 1 \\
377 & 150.10789 & 1.86154 & 22.75 & 1.358 & 4.5 $\pm$ 0.05 & 8.0 $\pm$ 0.28 & 44.7 & 4.72 & 1 \\
382 & 149.91953 & 2.34537 & 21.68 & 3.015 & 3.1 $\pm$ 0.01 & 8.3 $\pm$ 0.11 & 45.9 & 99.99 & 2 \\
389 & 149.63529 & 2.59886 & 22.17 & 2.536 & 5.0 $\pm$ 0.01 & 8.5 $\pm$ 0.11 & 45.6 & 6.84 & 2 \\
405 & 150.14709 & 2.71747 & 22.64 & 1.178 & 7.2 $\pm$ 0.03 & 8.5 $\pm$ 0.18 & 44.9 & 9.78 & 1 \\
410 & 150.45494 & 1.9674 & 23.85 & 3.477 & 4.1 $\pm$ 0.25 & 8.4 $\pm$ 0.5 & 45.8 & 99.99 & 2 \\
414 & 150.06922 & 2.23131 & 23.5 & 1.869 & 3.2 $\pm$ 0.01 & 7.8 $\pm$ 0.16 & 45.0 & 3.7 & 1 \\
417 & 149.50598 & 2.18535 & 22.02 & 3.225 & 7.3 $\pm$ 0.02 & 8.9 $\pm$ 0.14 & 45.7 & 4.03 & 2 \\
426 & 149.73592 & 2.02757 & 22.63 & 2.454 & 2.6 $\pm$ 1.08 & 8.1 $\pm$ 1.04 & 45.8 & 7.74 & 1 \\
432 & 150.08439 & 2.29048 & 22.6 & 2.101 & 9.4 $\pm$ 0.04 & 8.9 $\pm$ 0.2 & 45.1 & 4.51 & 1 \\
436 & 149.62421 & 2.18066 & 20.77 & 1.187 & 3.5 $\pm$ 0.01 & 8.2 $\pm$ 0.11 & 45.5 & 13.05 & 1 \\
\hline
\end{longtable}

==> zbhmass_latex_with_kimura2.tex <==
\begin{table*}[t]
 \centering
 \caption{The physical parameters of variability-selected AGNs with estimated $\MBH$}
  \label{bhmass-table1}
   \begin{tabular}{cccccccccc}
    \hline \hline
    varAGN ID & R.A.(J2000) & Dec.(J2000) & $i$-band & Redshift & $FWHM$ & $\MBH$ & $\Lbol$ & S/N & line \\
    \hline
      & [deg] & [deg] & [mag] &  & [$10^3\ \mathrm{km\ s^{-1}}$] & [$\Ms$] & [$\mathrm{erg\ s^{-1}}$] &  &  \\
    \hline
    (1) & (2) & (3) & (4) & (5) & (6) & (7) & (8) & (9) & (10) \\
\hline
&&&&X-det varAGN&&&&\\

% \endhead\hline\endfoot
1 & 150.74386 & 2.20245 & 22.71 & 1.618 & 6.4 $\pm$ 1.17 & 8.6 $\pm$ 1.08 & 45.3 & 6.63 & 2 \\
2 & 150.73557 & 2.19957 & 20.36 & 3.497 & 5.6 $\pm$ 0.03 & 8.8 $\pm$ 0.16 & 45.9 & 4.76 & 2 \\
7 & 150.78838 & 2.34399 & 19.82 & 1.964 & 4.6 $\pm$ 0.00 & 8.5 $\pm$ 0.07 & 45.8 & 7.46 & 2 \\
8 & 150.71511 & 2.48483 & 19.20 & 2.003 & 4.4 $\pm$ 0.00 & 8.5 $\pm$ 0.04 & 45.8 & 8.95 & 2 \\
12 & 150.65294 & 1.99685 & 19.52 & 1.518 & 3.0 $\pm$ 0.03 & 7.9 $\pm$ 0.19 & 45.1 & 8.03 & 1 \\
15 & 150.61224 & 1.99442 & 21.40 & 1.609 & 3.1 $\pm$ 0.16 & 7.8 $\pm$ 0.40 & 45.0 & 6.42 & 1 \\
16 & 150.57489 & 1.97677 & 20.98 & 1.541 & 4.9 $\pm$ 0.01 & 8.5 $\pm$ 0.08 & 45.5 & 11.98 & 1 \\
17 & 150.55903 & 2.10576 & 22.61 & 2.330 & 4.9 $\pm$ 0.14 & 8.8 $\pm$ 0.38 & 46.1 & 11.52 & 1 \\
19 & 150.70416 & 2.29746 & 21.59 & 2.740 & 3.5 $\pm$ 0.05 & 8.2 $\pm$ 0.22 & 45.5 & 99.99 & 2 \\
20 & 150.70801 & 2.29233 & 21.09 & 1.099 & 6.1 $\pm$ 0.00 & 8.5 $\pm$ 0.04 & 45.3 & 12.33 & 1 \\
22 & 150.58112 & 2.22107 & 21.92 & 2.023 & 6.3 $\pm$ 0.30 & 8.6 $\pm$ 0.55 & 45.3 & 5.9 & 1 \\
23 & 150.53187 & 2.18892 & 21.58 & 0.827 & 1.5 $\pm$ 0.02 & 7.0 $\pm$ 0.19 & 44.5 & 8.74 & 1 \\
24 & 150.60970 & 2.32311 & 20.44 & 1.295 & 2.4 $\pm$ 0.28 & 8.0 $\pm$ 0.53 & 45.9 & 15.3 & 1 \\
26 & 150.63020 & 2.45454 & 20.20 & 0.817 & 4.9 $\pm$ 0.13 & 8.0 $\pm$ 0.38 & 44.5 & 8.63 & 1 \\
27 & 150.55556 & 2.36917 & 23.29 & 1.640 & 4.2 $\pm$ 0.32 & 7.9 $\pm$ 0.59 & 44.7 & 3.33 & 2 \\
%28 & 150.59971 & 2.39823 & 20.77 & 2.836 & 2.4 $\pm$ 0.03 & 7.7 $\pm$ 0.18 & 45.3 & 3.9 & 2 \\
28 & 150.59971 & 2.39823 & 20.77 & 2.830 & 8.0 $\pm$ 0.33 & 8.8 $\pm$ 0.57 & 45.3 & 3.9 & 2 \\
30 & 150.61728 & 2.48275 & 22.59 & 2.733 & 7.9 $\pm$ 0.26 & 8.9 $\pm$ 0.51 & 45.5 & 4.25 & 2 \\
33 & 150.68315 & 2.57464 & 19.16 & 0.376 & 3.0 $\pm$ 0.01 & 7.4 $\pm$ 0.12 & 44.6 & 20.83 & 3 \\
34 & 150.63388 & 2.59371 & 19.13 & 0.657 & 2.8 $\pm$ 0.00 & 7.8 $\pm$ 0.05 & 45.2 & 21.78 & 1 \\
36 & 150.70554 & 2.62960 & 19.97 & 2.122 & 3.0 $\pm$ 0.02 & 8.3 $\pm$ 0.15 & 45.9 & 10.55 & 1 \\
37 & 150.63539 & 2.64991 & 21.04 & 1.223 & 5.2 $\pm$ 0.01 & 8.1 $\pm$ 0.15 & 44.7 & 5.64 & 1 \\
39 & 150.53932 & 2.54206 & 21.94 & 1.716 & 1.9 $\pm$ 0.38 & 7.4 $\pm$ 0.62 & 45.0 & 5.26 & 1 \\
43 & 150.55489 & 2.64105 & 21.58 & 1.142 & 6.5 $\pm$ 0.01 & 8.6 $\pm$ 0.09 & 45.2 & 12.06 & 1 \\
44 & 150.59735 & 2.61793 & 21.27 & 1.447 & 5.0 $\pm$ 0.01 & 8.3 $\pm$ 0.11 & 45.1 & 7.63 & 1 \\
46 & 150.44749 & 1.69569 & 22.04 & 2.160 & 2.3 $\pm$ 0.65 & 7.3 $\pm$ 0.80 & 44.4 & 99.99 & 1 \\
47 & 150.37654 & 1.71790 & 20.06 & 1.571 & 3.8 $\pm$ 0.09 & 8.2 $\pm$ 0.30 & 45.5 & 8.86 & 1 \\
51 & 150.49127 & 1.91029 & 21.95 & 2.234 & 2.0 $\pm$ 0.10 & 7.4 $\pm$ 0.36 & 44.8 & 3.31 & 1 \\
58 & 150.35942 & 1.93644 & 22.48 & 2.367 & 7.5 $\pm$ 1.47 & 8.6 $\pm$ 1.21 & 45.1 & 99.99 & 2 \\
60 & 150.43102 & 1.93527 & 21.47 & 2.171 & 6.3 $\pm$ 0.47 & 8.8 $\pm$ 0.69 & 45.6 & 9.02 & 1 \\
61 & 150.40096 & 1.91198 & 21.06 & 2.280 & 7.6 $\pm$ 0.08 & 9.1 $\pm$ 0.28 & 46.0 & 11.15 & 2 \\
63 & 150.44602 & 2.04351 & 20.82 & 1.171 & 8.1 $\pm$ 0.00 & 8.9 $\pm$ 0.06 & 45.4 & 13.07 & 1 \\
64 & 150.44368 & 2.04910 & 20.11 & 0.669 & 2.1 $\pm$ 0.01 & 7.5 $\pm$ 0.09 & 45.1 & 17.88 & 1 \\
66 & 150.42256 & 2.01415 & 21.79 & 2.283 & 4.5 $\pm$ 0.08 & 8.3 $\pm$ 0.28 & 45.3 & 6.12 & 1 \\
68 & 150.41834 & 2.08515 & 20.08 & 0.424 & 2.5 $\pm$ 0.07 & 7.0 $\pm$ 0.32 & 44.4 & 13.49 & 3 \\
70 & 150.45184 & 2.14481 & 20.64 & 1.298 & 1.7 $\pm$ 0.01 & 7.1 $\pm$ 0.17 & 44.7 & 5.63 & 1 \\
71 & 150.48437 & 2.16202 & 21.84 & 1.639 & 8.4 $\pm$ 0.01 & 8.9 $\pm$ 0.10 & 45.4 & 11.07 & 1 \\
73 & 150.44960 & 2.24643 & 20.67 & 0.882 & 3.0 $\pm$ 0.01 & 7.8 $\pm$ 0.11 & 45.1 & 11.88 & 1 \\
75 & 150.51907 & 2.32098 & 22.24 & 1.836 & 5.6 $\pm$ 0.02 & 8.6 $\pm$ 0.13 & 45.6 & 11.6 & 1 \\
77 & 150.36472 & 2.14380 & 23.24 & 3.328 & 2.7 $\pm$ 0.03 & 8.1 $\pm$ 0.18 & 45.9 & 4.43 & 2 \\
78 & 150.37824 & 2.19636 & 22.49 & 1.512 & 5.2 $\pm$ 0.02 & 8.5 $\pm$ 0.15 & 45.4 & 9.87 & 1 \\
79 & 150.34592 & 2.14752 & 20.74 & 1.256 & 2.9 $\pm$ 0.01 & 7.8 $\pm$ 0.11 & 45.1 & 99.99 & 1 \\
81 & 150.42223 & 2.17535 & 20.94 & 0.979 & 4.0 $\pm$ 0.01 & 8.2 $\pm$ 0.10 & 45.3 & 14.05 & 1 \\
83 & 150.37463 & 2.31020 & 23.05 & 2.155 & 8.1 $\pm$ 0.60 & 8.8 $\pm$ 0.77 & 45.3 & 5.28 & 2 \\
85 & 150.43817 & 2.41581 & 20.49 & 2.020 & 9.7 $\pm$ 0.01 & 8.9 $\pm$ 0.12 & 45.2 & 5.58 & 2 \\
87 & 150.49565 & 2.41256 & 21.62 & 1.369 & 5.7 $\pm$ 0.00 & 8.4 $\pm$ 0.07 & 45.1 & 9.27 & 1 \\
89 & 150.51157 & 2.40961 & 20.99 & 0.986 & 6.0 $\pm$ 0.04 & 8.4 $\pm$ 0.21 & 45.0 & 11.48 & 1 \\
\hline
\end{tabular}
\end{table*}

\begin{table*}[t]
 \centering
 \caption{Continued}
  % \label{bhmass-table1}
   \begin{tabular}{cccccccccc}
    \hline \hline
varAGN ID & R.A.(J2000) & Dec.(J2000) & $i$-band & Redshift & $FWHM$ & $\MBH$ & $\Lbol$ & S/N & line \\
\hline
  & [deg] & [deg] & [mag] &  & [$10^3\ \mathrm{km\ s^{-1}}$] & [$\Ms$] & [$\mathrm{erg\ s^{-1}}$] &  &  \\
\hline
(1) & (2) & (3) & (4) & (5) & (6) & (7) & (8) & (9) & (10) \\
\hline
91 & 150.49911 & 2.44491 & 19.03 & 2.030 & 4.6 $\pm$ 0.01 & 9.1 $\pm$ 0.11 & 46.9 & 21.1 & 1 \\
92 & 150.35363 & 2.34216 & 20.36 & 1.714 & 1.9 $\pm$ 0.42 & 7.8 $\pm$ 0.65 & 45.8 & 11.12 & 4 \\
93 & 150.40669 & 2.36546 & 21.80 & 2.037 & 2.8 $\pm$ 0.05 & 7.7 $\pm$ 0.23 & 45.1 & 99.99 & 2 \\
95 & 150.45360 & 2.52790 & 21.03 & 1.931 & 2.6 $\pm$ 0.05 & 7.8 $\pm$ 0.22 & 45.2 & 4.76 & 1 \\
96 & 150.45666 & 2.64811 & 20.36 & 2.050 & 4.5 $\pm$ 0.02 & 8.5 $\pm$ 0.15 & 45.7 & 9.11 & 1 \\
97 & 150.49762 & 2.65989 & 19.94 & 0.854 & 11.6 $\pm$ 0.00 & 9.1 $\pm$ 0.03 & 45.2 & 15.86 & 1 \\
99 & 150.38283 & 2.55977 & 22.94 & 2.068 & 7.1 $\pm$ 0.26 & 8.5 $\pm$ 0.52 & 45.0 & 3.98 & 2 \\
100 & 150.41596 & 2.52574 & 22.27 & 1.444 & 2.3 $\pm$ 0.01 & 7.5 $\pm$ 0.13 & 44.9 & 5.71 & 1 \\
101 & 150.35143 & 2.67822 & 21.15 & 2.754 & 8.0 $\pm$ 0.01 & 9.2 $\pm$ 0.10 & 46.1 & 8.86 & 2 \\
102 & 150.49077 & 2.77544 & 20.24 & 1.434 & 8.8 $\pm$ 0.01 & 9.4 $\pm$ 0.08 & 46.3 & 22.43 & 1 \\
105 & 150.38285 & 2.72363 & 22.35 & 2.053 & 8.6 $\pm$ 0.58 & 8.8 $\pm$ 0.76 & 45.3 & 6.24 & 2 \\
109 & 150.31993 & 1.68158 & 19.78 & 2.055 & 4.4 $\pm$ 0.01 & 8.6 $\pm$ 0.10 & 46.0 & 8.88 & 2 \\
113 & 150.30622 & 1.87518 & 23.31 & 1.759 & 4.1 $\pm$ 0.75 & 8.1 $\pm$ 0.86 & 45.2 & 99.99 & 2 \\
115 & 150.30889 & 1.91231 & 21.57 & 1.525 & 9.0 $\pm$ 0.90 & 9.1 $\pm$ 0.95 & 45.8 & 13.16 & 1 \\
119 & 150.24519 & 1.90011 & 20.01 & 1.560 & 2.6 $\pm$ 0.11 & 8.2 $\pm$ 0.33 & 46.0 & 15.43 & 1 \\
120 & 150.20823 & 1.87538 & 20.52 & 1.147 & 8.2 $\pm$ 0.03 & 8.6 $\pm$ 0.20 & 44.9 & 6.85 & 1 \\
121 & 150.24309 & 1.86912 & 20.58 & 2.027 & 3.5 $\pm$ 0.03 & 8.1 $\pm$ 0.18 & 45.4 & 6.33 & 1 \\
122 & 150.16179 & 1.87796 & 21.98 & 1.444 & 2.9 $\pm$ 0.00 & 7.9 $\pm$ 0.06 & 45.2 & 8.41 & 1 \\
124 & 150.25342 & 1.99661 & 21.93 & 1.171 & 8.2 $\pm$ 0.01 & 8.7 $\pm$ 0.11 & 45.0 & 7.79 & 1 \\
125 & 150.31186 & 1.97795 & 21.72 & 2.351 & 6.8 $\pm$ 0.24 & 8.8 $\pm$ 0.49 & 45.6 & 6.47 & 1 \\
126 & 150.28566 & 2.01459 & 21.20 & 2.654 & 5.6 $\pm$ 0.03 & 8.8 $\pm$ 0.19 & 46.0 & 7.33 & 2 \\
128 & 150.33439 & 2.06147 & 20.17 & 0.904 & 3.5 $\pm$ 0.02 & 7.8 $\pm$ 0.16 & 44.7 & 7.91 & 1 \\
129 & 150.30691 & 2.05384 & 23.60 & 2.005 & 6.2 $\pm$ 1.12 & 8.4 $\pm$ 1.06 & 45.0 & 4.04 & 2 \\
130 & 150.21637 & 1.98874 & 21.34 & 2.230 & 4.5 $\pm$ 0.14 & 8.6 $\pm$ 0.37 & 46.0 & 10.27 & 1 \\
131 & 150.18074 & 2.07598 & 22.87 & 2.994 & 5.8 $\pm$ 0.26 & 9.0 $\pm$ 0.51 & 46.3 & 99.99 & 2 \\
132 & 150.27217 & 2.23009 & 21.02 & 2.611 & 15.2 $\pm$ 0.06 & 9.9 $\pm$ 0.24 & 46.3 & 10.95 & 2 \\
133 & 150.30261 & 2.16108 & 20.23 & 1.817 & 4.5 $\pm$ 0.00 & 8.2 $\pm$ 0.08 & 45.1 & 5.05 & 1 \\
134 & 150.31652 & 2.24678 & 21.62 & 2.483 & 3.3 $\pm$ 0.12 & 8.0 $\pm$ 0.34 & 45.4 & 5.18 & 2 \\
136 & 150.15843 & 2.13957 & 20.14 & 1.829 & 5.7 $\pm$ 0.05 & 8.5 $\pm$ 0.24 & 45.3 & 6.12 & 1 \\
138 & 150.21469 & 2.20427 & 20.70 & 1.841 & 3.1 $\pm$ 0.01 & 8.2 $\pm$ 0.08 & 45.7 & 10.46 & 1 \\
139 & 150.19979 & 2.19085 & 20.92 & 1.515 & 8.5 $\pm$ 0.01 & 8.8 $\pm$ 0.08 & 45.2 & 7.45 & 1 \\
140 & 150.23628 & 2.28913 & 21.36 & 2.083 & 7.1 $\pm$ 0.13 & 8.4 $\pm$ 0.38 & 44.9 & 3.53 & 2 \\
142 & 150.25271 & 2.48638 & 21.15 & 2.040 & 7.3 $\pm$ 0.31 & 8.6 $\pm$ 0.56 & 45.1 & 5.22 & 1 \\
143 & 150.30809 & 2.43003 & 20.25 & 0.373 & 4.0 $\pm$ 0.04 & 7.3 $\pm$ 0.39 & 44.2 & 12.54 & 3 \\
144 & 150.29976 & 2.50687 & 21.03 & 1.503 & 1.8 $\pm$ 0.32 & 7.3 $\pm$ 0.57 & 45.1 & 8.07 & 4 \\
147 & 150.23182 & 2.36399 & 20.68 & 1.936 & 4.9 $\pm$ 0.01 & 8.5 $\pm$ 0.12 & 45.5 & 7.46 & 1 \\
149 & 150.24463 & 2.43227 & 20.63 & 0.696 & 3.3 $\pm$ 0.06 & 7.4 $\pm$ 0.28 & 44.6 & 11.71 & 3 \\
150 & 150.20902 & 2.43846 & 21.00 & 3.715 & 8.5 $\pm$ 0.01 & 9.3 $\pm$ 0.11 & 46.3 & 99.99 & 2 \\
151 & 150.20887 & 2.48189 & 19.71 & 3.333 & 4.9 $\pm$ 0.00 & 8.6 $\pm$ 0.05 & 45.7 & 4.44 & 2 \\
152 & 150.29252 & 2.54507 & 21.48 & 2.653 & 6.0 $\pm$ 0.02 & 8.9 $\pm$ 0.13 & 46.1 & 9.45 & 2 \\
153 & 150.32383 & 2.55258 & 22.83 & 1.002 & 1.8 $\pm$ 0.12 & 7.1 $\pm$ 0.36 & 44.9 & 9.99 & 4 \\
154 & 150.31791 & 2.60207 & 20.86 & 0.958 & 3.9 $\pm$ 0.18 & 8.2 $\pm$ 0.42 & 45.4 & 13.66 & 1 \\
155 & 150.33446 & 2.56146 & 19.86 & 1.836 & 3.2 $\pm$ 0.01 & 8.0 $\pm$ 0.12 & 45.3 & 6.98 & 1 \\
158 & 150.29780 & 2.67347 & 21.83 & 1.603 & 12.1 $\pm$ 1.39 & 8.9 $\pm$ 1.18 & 44.8 & 5.37 & 1 \\
160 & 150.16384 & 2.59765 & 21.91 & 1.589 & 4.7 $\pm$ 0.05 & 8.2 $\pm$ 0.22 & 45.0 & 5.55 & 1 \\
162 & 150.23083 & 2.57815 & 19.58 & 1.402 & 6.9 $\pm$ 0.01 & 8.9 $\pm$ 0.09 & 45.7 & 13.82 & 1 \\
165 & 150.29771 & 2.73879 & 23.22 & 1.954 & 3.8 $\pm$ 0.06 & 8.0 $\pm$ 0.24 & 45.1 & 5.47 & 2 \\
\hline
\end{tabular}
\end{table*}


\begin{table*}[t]
 \centering
 \caption{Continued}
  % \label{bhmass-table1}
   \begin{tabular}{cccccccccc}
    \hline \hline
varAGN ID & R.A.(J2000) & Dec.(J2000) & $i$-band & Redshift & $FWHM$ & $\MBH$ & $\Lbol$ & S/N & line \\
\hline
  & [deg] & [deg] & [mag] &  & [$10^3\ \mathrm{km\ s^{-1}}$] & [$\Ms$] & [$\mathrm{erg\ s^{-1}}$] &  &  \\
\hline
(1) & (2) & (3) & (4) & (5) & (6) & (7) & (8) & (9) & (10) \\
\hline
166 & 150.33854 & 2.77670 & 22.94 & 2.126 & 4.5 $\pm$ 0.44 & 8.4 $\pm$ 0.66 & 45.6 & 9.26 & 2 \\
168 & 150.25135 & 2.73714 & 20.76 & 2.167 & 4.7 $\pm$ 0.05 & 8.5 $\pm$ 0.22 & 45.6 & 7.5 & 1 \\
169 & 150.16706 & 2.76891 & 21.92 & 2.388 & 6.3 $\pm$ 0.39 & 8.4 $\pm$ 0.63 & 45.1 & 3.49 & 2 \\
170 & 150.05185 & 1.68279 & 20.17 & 2.276 & 6.1 $\pm$ 0.00 & 8.8 $\pm$ 0.06 & 45.8 & 8.92 & 2 \\
171 & 149.99161 & 1.72432 & 20.21 & 1.625 & 4.0 $\pm$ 0.11 & 8.2 $\pm$ 0.33 & 45.3 & 7.67 & 1 \\
172 & 150.13175 & 1.79944 & 20.84 & 1.679 & 8.6 $\pm$ 0.02 & 9.2 $\pm$ 0.13 & 45.9 & 12.24 & 1 \\
173 & 150.12456 & 1.80983 & 22.71 & 1.358 & 2.1 $\pm$ 0.32 & 7.6 $\pm$ 0.56 & 45.1 & 99.99 & 1 \\
174 & 150.10166 & 1.84837 & 19.81 & 1.666 & 2.2 $\pm$ 0.01 & 7.6 $\pm$ 0.12 & 45.3 & 7.5 & 4 \\
176 & 150.08145 & 1.90601 & 23.08 & 1.817 & 4.5 $\pm$ 0.53 & 7.7 $\pm$ 0.85 & 44.2 & 3.68 & 2 \\
179 & 149.98874 & 1.93244 & 22.58 & 2.405 & 5.0 $\pm$ 0.23 & 8.2 $\pm$ 0.48 & 45.0 & 3.51 & 2 \\
183 & 149.99527 & 2.00665 & 21.97 & 1.033 & 1.5 $\pm$ 0.26 & 6.9 $\pm$ 0.52 & 44.8 & 7.3 & 4 \\
184 & 150.00440 & 2.03891 & 21.55 & 3.499 & 4.2 $\pm$ 0.01 & 8.3 $\pm$ 0.08 & 45.5 & 3.66 & 2 \\
185 & 150.05894 & 2.01516 & 19.63 & 2.498 & 3.5 $\pm$ 0.00 & 8.5 $\pm$ 0.06 & 46.1 & 9.29 & 2 \\
186 & 149.99176 & 2.13195 & 22.85 & 2.131 & 5.3 $\pm$ 0.69 & 8.5 $\pm$ 0.83 & 45.3 & 4.36 & 1 \\
190 & 150.13803 & 2.29165 & 17.56 & 0.185 & 0.9 $\pm$ 0.00 & 5.8 $\pm$ 0.67 & 43.8 & 15.68 & 4 \\
195 & 149.99391 & 2.30143 & 19.89 & 1.796 & 6.1 $\pm$ 0.02 & 8.8 $\pm$ 0.14 & 45.9 & 11.83 & 1 \\
196 & 150.00447 & 2.23711 & 21.61 & 1.406 & 3.3 $\pm$ 0.00 & 8.1 $\pm$ 0.05 & 45.5 & 10.82 & 1 \\
197 & 150.06456 & 2.32902 & 21.85 & 2.450 & 6.3 $\pm$ 0.06 & 8.6 $\pm$ 0.26 & 45.3 & 4.05 & 1 \\
198 & 150.09156 & 2.39905 & 21.75 & 2.470 & 3.7 $\pm$ 0.09 & 8.5 $\pm$ 0.30 & 46.0 & 8.97 & 2 \\
199 & 150.12369 & 2.35825 & 20.03 & 0.728 & 1.8 $\pm$ 0.16 & 7.1 $\pm$ 0.41 & 44.9 & 12.43 & 3 \\
201 & 150.00423 & 2.38915 & 23.28 & 1.846 & 1.9 $\pm$ 0.04 & 7.4 $\pm$ 0.22 & 45.0 & 4.7 & 1 \\
203 & 150.05873 & 2.47739 & 20.62 & 1.258 & 5.2 $\pm$ 0.01 & 8.4 $\pm$ 0.09 & 45.2 & 9.94 & 1 \\
207 & 150.10447 & 2.69123 & 21.21 & 1.881 & 2.8 $\pm$ 0.07 & 8.1 $\pm$ 0.26 & 45.7 & 11.3 & 1 \\
209 & 150.12689 & 2.62654 & 21.68 & 1.839 & 2.6 $\pm$ 0.04 & 8.0 $\pm$ 0.20 & 45.7 & 10.89 & 1 \\
211 & 150.04526 & 2.68849 & 21.78 & 1.438 & 2.5 $\pm$ 0.07 & 7.8 $\pm$ 0.27 & 45.4 & 12.39 & 1 \\
212 & 150.04251 & 2.62916 & 20.44 & 1.569 & 7.5 $\pm$ 0.02 & 8.9 $\pm$ 0.15 & 45.7 & 11.05 & 1 \\
214 & 150.06065 & 2.64796 & 20.87 & 0.437 & 3.5 $\pm$ 0.02 & 7.0 $\pm$ 1.2 & 44.0 & 6.13 & 3 \\
215 & 150.03066 & 2.67873 & 21.46 & 1.943 & 10.0 $\pm$ 0.77 & 8.9 $\pm$ 0.88 & 45.2 & 5.57 & 1 \\
222 & 149.81688 & 1.84673 & 20.76 & 1.035 & 8.3 $\pm$ 0.02 & 8.6 $\pm$ 0.14 & 44.9 & 10.64 & 1 \\
224 & 149.82193 & 1.83866 & 20.93 & 1.351 & 4.8 $\pm$ 0.01 & 8.4 $\pm$ 0.09 & 45.3 & 10.84 & 1 \\
227 & 149.79179 & 1.87287 & 22.21 & 1.566 & 4.2 $\pm$ 0.03 & 8.0 $\pm$ 0.20 & 44.8 & 5.33 & 1 \\
228 & 149.92256 & 1.97922 & 22.24 & 2.508 & 3.6 $\pm$ 0.11 & 8.2 $\pm$ 0.32 & 45.5 & 5.58 & 2 \\
230 & 149.95773 & 2.00310 & 20.82 & 1.806 & 5.6 $\pm$ 0.02 & 8.5 $\pm$ 0.14 & 45.3 & 4.96 & 1 \\
231 & 149.90955 & 2.08058 & 20.35 & 2.802 & 4.3 $\pm$ 0.00 & 8.4 $\pm$ 0.05 & 45.6 & 5.4 & 2 \\
232 & 149.89793 & 2.09392 & 21.49 & 1.921 & 3.0 $\pm$ 0.05 & 8.1 $\pm$ 0.23 & 45.6 & 8.24 & 1 \\
235 & 149.89510 & 2.04721 & 21.78 & 2.198 & 4.3 $\pm$ 0.01 & 8.3 $\pm$ 0.08 & 45.3 & 5.32 & 1 \\
236 & 149.81421 & 2.01633 & 22.48 & 1.359 & 8.3 $\pm$ 1.03 & 8.8 $\pm$ 1.02 & 45.3 & 9.16 & 1 \\
238 & 149.82269 & 2.08965 & 21.87 & 2.051 & 10.4 $\pm$ 0.01 & 9.2 $\pm$ 0.08 & 45.6 & 7.64 & 1 \\
239 & 149.91244 & 2.20032 & 20.30 & 0.686 & 1.5 $\pm$ 0.03 & 6.9 $\pm$ 0.24 & 44.5 & 7.85 & 1 \\
240 & 149.89483 & 2.17443 & 21.55 & 1.312 & 6.7 $\pm$ 0.04 & 8.6 $\pm$ 0.2 & 45.1 & 7.15 & 1 \\
241 & 149.89540 & 2.23947 & 20.70 & 1.729 & 3.5 $\pm$ 0.11 & 7.9 $\pm$ 0.35 & 45.0 & 3.86 & 1 \\
242 & 149.78190 & 2.13906 & 18.54 & 0.354 & 6.0 $\pm$ 0.11 & 8.1 $\pm$ 0.35 & 44.3 & 16.43 & 1 \\
244 & 149.78977 & 2.32120 & 20.07 & 0.378 & 1.9 $\pm$ 0.02 & 6.8 $\pm$ 0.27 & 44.4 & 12.15 & 4 \\
249 & 149.91977 & 2.32742 & 20.27 & 1.454 & 7.3 $\pm$ 0.00 & 9.2 $\pm$ 0.04 & 46.3 & 19.79 & 1 \\
251 & 149.91694 & 2.38518 & 19.78 & 1.131 & 3.3 $\pm$ 0.00 & 8.0 $\pm$ 0.04 & 45.3 & 12.09 & 1 \\
252 & 149.88334 & 2.34673 & 21.46 & 1.021 & 3.0 $\pm$ 0.10 & 7.6 $\pm$ 0.34 & 44.7 & 6.85 & 1 \\
253 & 149.88102 & 2.45083 & 21.51 & 1.313 & 2.8 $\pm$ 0.01 & 7.5 $\pm$ 0.39 & 44.5 & 3.46 & 1 \\
\hline
\end{tabular}
\end{table*}


\begin{table*}[t]
 \centering
 \caption{Continued}
  % \label{bhmass-table1}
   \begin{tabular}{cccccccccc}
    \hline \hline
varAGN ID & R.A.(J2000) & Dec.(J2000) & $i$-band & Redshift & $FWHM$ & $\MBH$ & $\Lbol$ & S/N & line \\
\hline
  & [deg] & [deg] & [mag] &  & [$10^3\ \mathrm{km\ s^{-1}}$] & [$\Ms$] & [$\mathrm{erg\ s^{-1}}$] &  &  \\
\hline
(1) & (2) & (3) & (4) & (5) & (6) & (7) & (8) & (9) & (10) \\
\hline
256 & 149.95563 & 2.50204 & 22.38 & 1.458 & 8.1 $\pm$ 0.00 & 8.9 $\pm$ 0.05 & 45.5 & 10.74 & 1 \\
258 & 149.81293 & 2.34546 & 21.54 & 1.812 & 4.7 $\pm$ 0.09 & 8.1 $\pm$ 0.33 & 44.9 & 3.75 & 1 \\
260 & 149.87071 & 2.41727 & 21.93 & 1.528 & 5.1 $\pm$ 0.02 & 8.1 $\pm$ 0.21 & 44.8 & 4.52 & 1 \\
262 & 149.86806 & 2.33069 & 20.55 & 1.478 & 4.3 $\pm$ 0.00 & 8.2 $\pm$ 0.04 & 45.2 & 8.32 & 1 \\
263 & 149.87184 & 2.34286 & 21.55 & 1.743 & 3.7 $\pm$ 0.20 & 8.0 $\pm$ 0.46 & 45.0 & 4.84 & 1 \\
265 & 149.91067 & 2.55465 & 19.96 & 0.753 & 6.4 $\pm$ 0.25 & 7.9 $\pm$ 1.39 & 44.0 & 3.41 & 1 \\
266 & 149.87591 & 2.69026 & 21.39 & 2.169 & 4.8 $\pm$ 0.02 & 8.5 $\pm$ 0.14 & 45.7 & 9.68 & 2 \\
269 & 149.92540 & 2.68423 & 20.28 & 1.779 & 3.6 $\pm$ 0.01 & 8.0 $\pm$ 0.13 & 45.1 & 4.35 & 2 \\
270 & 149.78564 & 2.55479 & 22.32 & 1.798 & 4.6 $\pm$ 0.41 & 8.3 $\pm$ 0.64 & 45.3 & 7.65 & 1 \\
272 & 149.81144 & 2.55798 & 23.03 & 2.152 & 4.5 $\pm$ 0.52 & 8.1 $\pm$ 0.72 & 45.0 & 4.62 & 2 \\
273 & 149.86032 & 2.54475 & 22.77 & 1.596 & 8.5 $\pm$ 0.02 & 8.9 $\pm$ 0.16 & 45.4 & 9.24 & 1 \\
274 & 149.80800 & 2.64568 & 21.19 & 2.082 & 7.7 $\pm$ 0.05 & 9.0 $\pm$ 0.23 & 45.8 & 9.9 & 1 \\
279 & 149.68747 & 1.81266 & 22.58 & 1.214 & 7.7 $\pm$ 0.02 & 8.6 $\pm$ 0.16 & 45.0 & 8.36 & 1 \\
280 & 149.64996 & 1.86587 & 19.48 & 2.935 & 4.3 $\pm$ 0.13 & 8.4 $\pm$ 0.36 & 45.6 & 5.16 & 2 \\
281 & 149.67418 & 1.88837 & 19.97 & 1.770 & 8.8 $\pm$ 0.07 & 9.3 $\pm$ 0.27 & 46.2 & 14.51 & 1 \\
282 & 149.71561 & 2.01652 & 23.08 & 2.686 & 2.1 $\pm$ 0.00 & 7.7 $\pm$ 0.07 & 45.5 & 4.86 & 2 \\
283 & 149.74451 & 2.02752 & 19.39 & 2.448 & 8.9 $\pm$ 0.03 & 9.5 $\pm$ 0.16 & 46.6 & 13.33 & 2 \\
284 & 149.75359 & 2.12563 & 22.36 & 1.951 & 1.8 $\pm$ 0.01 & 7.1 $\pm$ 0.08 & 44.4 & 99.99 & 1 \\
286 & 149.66361 & 2.08522 & 20.18 & 1.220 & 2.7 $\pm$ 0.01 & 7.8 $\pm$ 0.08 & 45.1 & 10.56 & 1 \\
288 & 149.73896 & 2.22069 & 20.37 & 1.024 & 9.8 $\pm$ 0.02 & 9.7 $\pm$ 0.14 & 46.8 & 31.53 & 1 \\
289 & 149.71125 & 2.14515 & 20.31 & 1.538 & 8.9 $\pm$ 0.45 & 8.7 $\pm$ 0.67 & 44.9 & 99.99 & 1 \\
293 & 149.66680 & 2.28643 & 21.02 & 1.028 & 5.3 $\pm$ 0.07 & 8.3 $\pm$ 0.27 & 45.0 & 11.03 & 1 \\
295 & 149.76348 & 2.33414 & 20.99 & 1.137 & 6.8 $\pm$ 0.02 & 8.4 $\pm$ 0.19 & 44.7 & 6.31 & 1 \\
297 & 149.69877 & 2.44124 & 21.23 & 1.516 & 3.4 $\pm$ 0.86 & 8.2 $\pm$ 0.93 & 45.7 & 8.92 & 4 \\
298 & 149.70583 & 2.41980 & 20.39 & 1.122 & 12.2 $\pm$ 0.00 & 9.6 $\pm$ 0.05 & 46.1 & 22.99 & 1 \\
299 & 149.73852 & 2.43387 & 21.52 & 2.097 & 2.8 $\pm$ 0.02 & 7.7 $\pm$ 0.23 & 44.9 & 3.1 & 1 \\
300 & 149.77692 & 2.44428 & 22.41 & 4.164 & 6.7 $\pm$ 0.25 & 8.9 $\pm$ 0.50 & 45.7 & 99.99 & 2 \\
303 & 149.62804 & 2.45950 & 22.16 & 1.167 & 5.2 $\pm$ 0.02 & 8.1 $\pm$ 0.18 & 44.7 & 6.93 & 1 \\
304 & 149.61116 & 2.47171 & 20.59 & 0.693 & 0.7 $\pm$ 0.06 & 6.3 $\pm$ 0.25 & 44.9 & 13.87 & 3 \\
305 & 149.70361 & 2.57810 & 20.48 & 1.545 & 5.6 $\pm$ 0.02 & 8.6 $\pm$ 0.15 & 45.6 & 12.2 & 1 \\
307 & 149.72134 & 2.54001 & 21.57 & 1.738 & 4.6 $\pm$ 0.16 & 8.2 $\pm$ 0.40 & 45.1 & 4.95 & 1 \\
312 & 149.58664 & 2.03712 & 20.48 & 1.850 & 5.6 $\pm$ 0.00 & 8.9 $\pm$ 0.05 & 46.2 & 13.63 & 1 \\
313 & 149.57351 & 2.02367 & 21.52 & 2.808 & 1.0 $\pm$ 0.05 & 7.1 $\pm$ 0.23 & 45.5 & 5.32 & 2 \\
315 & 149.56469 & 1.97790 & 20.97 & 1.688 & 4.3 $\pm$ 0.02 & 8.5 $\pm$ 0.13 & 45.9 & 10.79 & 1 \\
318 & 149.50675 & 2.07472 & 22.34 & 1.226 & 6.8 $\pm$ 0.02 & 8.6 $\pm$ 0.14 & 45.2 & 7.81 & 1 \\
321 & 149.57310 & 2.32739 & 21.06 & 0.731 & 3.6 $\pm$ 0.04 & 7.4 $\pm$ 0.27 & 44.5 & 10.44 & 3 \\
327 & 150.42196 & 2.38551 & 23.34 & 1.516 & 3.1 $\pm$ 1.67 & 7.9 $\pm$ 1.29 & 45.3 & 8.07 & 4 \\
329 & 150.34122 & 1.76125 & 23.72 & 2.930 & 4.4 $\pm$ 0.09 & 8.0 $\pm$ 0.30 & 44.8 & 99.99 & 2 \\
344 & 149.79629 & 2.55944 & 22.41 & 1.548 & 4.9 $\pm$ 1.07 & 8.2 $\pm$ 1.04 & 45.0 & 5.44 & 2 \\
351 & 150.32723 & 1.92860 & 20.07 & 0.528 & 3.1 $\pm$ 0.00 & 7.1 $\pm$ 0.49 & 44.2 & 7.68 & 3 \\
369 & 150.34772 & 2.39099 & 22.41 & 1.847 & 6.9 $\pm$ 0.02 & 8.7 $\pm$ 0.16 & 45.4 & 6.52 & 1 \\
377 & 150.10789 & 1.86154 & 22.75 & 1.358 & 4.5 $\pm$ 0.05 & 8.0 $\pm$ 0.28 & 44.7 & 4.72 & 1 \\
382 & 149.91953 & 2.34537 & 21.68 & 3.015 & 3.1 $\pm$ 0.01 & 8.3 $\pm$ 0.11 & 45.9 & 99.99 & 2 \\
389 & 149.63529 & 2.59886 & 22.17 & 2.536 & 5.0 $\pm$ 0.01 & 8.5 $\pm$ 0.11 & 45.6 & 6.84 & 2 \\
405 & 150.14709 & 2.71747 & 22.64 & 1.178 & 7.2 $\pm$ 0.03 & 8.5 $\pm$ 0.18 & 44.9 & 9.78 & 1 \\
410 & 150.45494 & 1.96740 & 23.85 & 3.477 & 4.1 $\pm$ 0.25 & 8.4 $\pm$ 0.50 & 45.8 & 99.99 & 2 \\
414 & 150.06922 & 2.23131 & 23.50 & 1.869 & 3.2 $\pm$ 0.01 & 7.8 $\pm$ 0.16 & 45.0 & 3.7 & 1 \\
\hline
\end{tabular}
\end{table*}

\begin{table*}[t]
 \centering
 \caption{Continued}
  % \label{bhmass-table1}
   \begin{tabular}{cccccccccc}
    \hline \hline
varAGN ID & R.A.(J2000) & Dec.(J2000) & $i$-band & Redshift & $FWHM$ & $\MBH$ & $\Lbol$ & S/N & line \\
\hline
  & [deg] & [deg] & [mag] &  & [$10^3\ \mathrm{km\ s^{-1}}$] & [$\Ms$] & [$\mathrm{erg\ s^{-1}}$] &  &  \\
\hline
(1) & (2) & (3) & (4) & (5) & (6) & (7) & (8) & (9) & (10) \\
\hline
417 & 149.50598 & 2.18535 & 22.02 & 3.225 & 7.3 $\pm$ 0.02 & 8.9 $\pm$ 0.14 & 45.7 & 4.03 & 2 \\
426 & 149.73592 & 2.02757 & 22.63 & 2.454 & 2.6 $\pm$ 1.08 & 8.1 $\pm$ 1.04 & 45.8 & 7.74 & 1 \\
432 & 150.08439 & 2.29048 & 22.60 & 2.101 & 9.4 $\pm$ 0.04 & 8.9 $\pm$ 0.20 & 45.1 & 4.51 & 1 \\
436 & 149.62421 & 2.18066 & 20.77 & 1.187 & 3.5 $\pm$ 0.01 & 8.2 $\pm$ 0.11 & 45.5 & 13.05 & 1 \\
\hline
\hline
&&&&X-undet varAGN&&&&\\
56 & 150.42931 & 1.82558 & 21.74 & 2.084 & 5.9 $\pm$ 0.17 & 8.4 $\pm$ 0.42 & 45.0 & 0 & 2 \\
108 & 150.36187 & 2.77911 & 22.54 & 2.537 & 6.5 $\pm$ 0.51 & 8.5 $\pm$ 0.71 & 45.2 & 0 & 2 \\
113 & 150.30622 & 1.87518 & 23.31 & 1.755 & 2.2 $\pm$ 0.08 & 7.6 $\pm$ 0.28 & 45.2 & 0 & 1 \\
114 & 150.33866 & 1.92814 & 22.89 & 1.608 & 4.0 $\pm$ 0.06 & 7.7 $\pm$ 0.37 & 44.3 & 2.16 & 1 \\
146 & 150.21078 & 2.39146 & 22.67 & 3.086 & 8.8 $\pm$ 0.68 & 8.8 $\pm$ 0.82 & 45.1 & 0 & 2 \\
177 & 150.02548 & 1.87768 & 22.51 & 1.801 & 3.3 $\pm$ 0.24 & 7.7 $\pm$ 0.49 & 44.8 & 0 & 2 \\
204 & 149.97694 & 2.48667 & 22.75 & 2.089 & 6.4 $\pm$ 0.02 & 8.7 $\pm$ 0.16 & 45.4 & 0 & 1 \\
248 & 149.85156 & 2.27640 & 23.30 & 3.369 & 7.8 $\pm$ 0.31 & 8.6 $\pm$ 0.56 & 45.1 & 0 & 2 \\
259 & 149.83285 & 2.38468 & 21.84 & 2.249 & 5.4 $\pm$ 0.79 & 8.5 $\pm$ 0.89 & 45.4 & 0 & 1 \\
264 & 149.84815 & 2.37424 & 20.52 & 2.724 & 9.2 $\pm$ 0.29 & 9.2 $\pm$ 0.54 & 45.8 & 2.84 & 2 \\
%264 & 149.84815 & 2.37424 & 20.52 & 2.735 & 5.2 $\pm$ 0.0 & 8.3 $\pm$ 0.07 & 45.1 & 2.87 & 2 \\
289 & 149.71125 & 2.14515 & 20.31 & 1.530 & 3.1 $\pm$ 0.00 & 7.8 $\pm$ 0.18 & 44.9 & 0 & 1 \\
342 & 149.84577 & 2.48161 & 23.50 & 3.360 & 6.3 $\pm$ 0.01 & 8.7 $\pm$ 0.11 & 45.5 & 0 & 2 \\
%431 & 150.19265 & 2.21984 & 23.68 & 3.09 & 4.7 $\pm$ 0.01 & 8.2 $\pm$ 0.2 & 45.1 & 2.33 & 2 \\
% \hline
354 & 150.26174 & 2.11664 & 21.15 & 2.537 & 7.9 $\pm$ 0.16 & 9.0 $\pm$ 0.40 & 45.7 & 0 & 2 \\
410 & 150.45494 & 1.96740 & 23.85 & 3.471 & 4.8 $\pm$ 0.02 & 8.6 $\pm$ 0.13 & 45.8 & 0 & 2 \\
431 & 150.19265 & 2.21984 & 23.68 & 3.084 & 7.5 $\pm$ 0.32 & 8.6 $\pm$ 0.61 & 45.0 & 2.33 & 2 \\
472 & 150.06852 & 2.40944 & 22.56 & 1.565 & 1.4 $\pm$ 0.10 & 6.6 $\pm$ 0.10 & 44.0 & 0 & 1 \\
485 & 150.09361 & 2.23721 & 22.31 & 1.175 & 2.6 $\pm$ 0.48 & 7.4 $\pm$ 0.48 & 44.5 & 0 & 1 \\
  \hline
\end{tabular}
\begin{tablenotes}
\item[](1)(2)(3)(4) ID, Right Ascension, Declination and $i$-band AB magnitude are taken from \citet{kimura_properties_2020}.  (5) spectroscopic redshift (6)(7) the FWHM of the broad line, mass of the SMBH (8) bolometric luminosity converted from hard X-ray luminosity and SED fitting result for X-ray detected AGNs and  X-ray undetected AGNs respectively. (9) Signal to noise ratio of hard X-ray in the Chandra COSMOS Legacy Survey \citep{laigle2016cosmos2015,marchesi2016chandra} (10) the label of the broad lines we use to estimate $\MBH$, 1 :$\Mgtwo$, 2: $\Cfour$, 3: $\Hb$, 4: $\Ha$.
\end{tablenotes}
\end{table*}

==> zbhmass_latex_with_kimura_sunundrer.tex <==
\begin{longtable}{|c|c|c|c|c|c|c|c|c|c|}
\hline
lsid & kimuracol2 & kimuracol3 & lz & lvvar $\pm$ lvvarerr & lsbhmassx $\pm$ ltbherr & lsbolx & lsxsn & lline \\
\hline
113 & 150.30622 & 1.87518 & 23.31 & 1.755 & 2.2 $\pm$ 0.08 & 7.6 $\pm$ 0.28 & 45.2 & 99.99 & 1 \\
114 & 150.33866 & 1.92814 & 22.89 & 1.608 & 4.0 $\pm$ 0.06 & 7.7 $\pm$ 0.37 & 44.3 & 2.16 & 1 \\
204 & 149.97694 & 2.48667 & 22.75 & 2.089 & 6.4 $\pm$ 0.02 & 8.7 $\pm$ 0.16 & 45.4 & 99.99 & 1 \\
264 & 149.84815 & 2.37424 & 20.52 & 2.735 & 5.2 $\pm$ 0.0 & 8.3 $\pm$ 0.07 & 45.1 & 2.87 & 2 \\
289 & 149.71125 & 2.14515 & 20.31 & 1.53 & 3.1 $\pm$ 0.0 & 7.8 $\pm$ 0.18 & 44.9 & 99.99 & 1 \\
342 & 149.84577 & 2.48161 & 23.5 & 3.36 & 6.3 $\pm$ 0.01 & 8.7 $\pm$ 0.11 & 45.5 & 99.99 & 2 \\
410 & 150.45494 & 1.9674 & 23.85 & 3.471 & 4.8 $\pm$ 0.02 & 8.6 $\pm$ 0.13 & 45.8 & 99.99 & 2 \\
431 & 150.19265 & 2.21984 & 23.68 & 3.09 & 4.7 $\pm$ 0.01 & 8.2 $\pm$ 0.2 & 45.1 & 2.33 & 2 \\
\hline
\end{longtable}

==> zbhmass_latex_with_kimura_xundet.tex <==
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
\hline
xsid & kimuracol2 & kimuracol3 & lz & lvvar $\pm$ lvvarerr & lsbhmassx $\pm$ ltbherr & lsbolx & lsxsn & lline \\
\hline
56 & 150.42931 & 1.82558 & 21.74 & 2.084 & 5.9 $\pm$ 0.17 & 8.4 $\pm$ 0.42 & 8.7 & 0 & 2 \\
108 & 150.36187 & 2.77911 & 22.54 & 2.537 & 6.5 $\pm$ 0.51 & 8.5 $\pm$ 0.71 & 8.7 & 0 & 2 \\
146 & 150.21078 & 2.39146 & 22.67 & 3.086 & 8.8 $\pm$ 0.68 & 8.8 $\pm$ 0.82 & 8.7 & 0 & 2 \\
177 & 150.02548 & 1.87768 & 22.51 & 1.801 & 3.3 $\pm$ 0.24 & 7.7 $\pm$ 0.49 & 8.7 & 0 & 2 \\
248 & 149.85156 & 2.2764 & 23.3 & 3.369 & 7.8 $\pm$ 0.31 & 8.6 $\pm$ 0.56 & 8.7 & 0 & 2 \\
259 & 149.83285 & 2.38468 & 21.84 & 2.249 & 5.4 $\pm$ 0.79 & 8.5 $\pm$ 0.89 & 45.4 & 0 & 1 \\
264 & 149.84815 & 2.37424 & 20.52 & 2.724 & 9.2 $\pm$ 0.29 & 9.2 $\pm$ 0.54 & 8.7 & 0 & 2 \\
354 & 150.26174 & 2.11664 & 21.15 & 2.537 & 7.9 $\pm$ 0.16 & 9.0 $\pm$ 0.4 & 8.7 & 0 & 2 \\
431 & 150.19265 & 2.21984 & 23.68 & 3.084 & 7.5 $\pm$ 0.32 & 8.6 $\pm$ 0.61 & 8.7 & 0 & 2 \\
472 & 150.06852 & 2.40944 & 22.56 & 1.565 & 1.4 $\pm$ 0.1 & 6.6 $\pm$ 0.1 & 44.0 & 0 & 1 \\
485 & 150.09361 & 2.23721 & 22.31 & 1.175 & 2.6 $\pm$ 0.48 & 7.4 $\pm$ 0.48 & 44.5 & 0 & 1 \\
\hline
\end{tabular}
